Polarities & Focussing: a journey from Realisability to Automated Reasoning

This dissertation explores the roles of polarities and focussing in various aspects of Computational Logic. These concepts play a key role in the the interpretation of proofs as programs, a.k.a. the Curry-Howard correspondence, in the context of classical logic. Arising from linear logic, they allow the construction of meaningful semantics for cut-elimination in classical logic, some of which relate to the Call-by-Name and Call-by-Value disciplines of functional programming. The first part of this dissertation provides an introduction to these interpretations, highlighting the roles of polarities and focussing. For instance: proofs of positive formulae provide structured data, while proofs of negative formulae consume such data; focussing allows the description of the interaction between the two kinds of proofs as pure pattern-matching. This idea is pushed further in the second part of this dissertation, and connected to realisability semantics, where the structured data is interpreted algebraically, and the consumption of such data is modelled with the use of an orthogonality relation. Most of this part has been proved in the Coq proof assistant. Polarities and focussing were also introduced with applications to logic programming in mind, where computation is proof-search. In the third part of this dissertation, we push this idea further by exploring the roles that these concepts can play in other applications of proof-search, such as theorem proving and more particularly automated reasoning. We use these concepts to describe the main algorithm of SAT-solvers and SMT-solvers: DPLL. We then describe the implementation of a proof-search engine called Psyche. Its architecture, based on the concept of focussing, offers a platform where smart techniques from automated reasoning (or a user interface) can safely and trustworthily be implemented via the use of an API.

==> 2_Ortho/lecture5.tex <==
\Lectureslide[V]{Classical Realisability}

\minitoc 

\Slide[Overview]{
  \strut
  \vfil
  \dis1{\columns{
      \column[.85]{
        \(
        \infer{\mbox{Computational interpretation of logic}}
        {
          \mbox{Proof-Search}
          \quad
          \infer{\mbox{Curry-Howard corr.}}
          {
            \disloc2{
              \iinfer{[]\mbox{Typing}}{
                \disloc3{
                  \iinfer{[]t\col A}{
                    \iinfer{[]\mbox{$t$ \emph{is of type} $A$}}{
                      \disloc4{\mbox{def.\ by induction on $t$}}
                    }
                  }
                }
              }
            }
            \disloc2{\iinfer{[]\mbox{Realisability}}{
                \disloc3{
                  \iinfer{[]t\Vdash A}{
                    \iinfer{[]\mbox{$t$ \emph{realises} $A$}}{
                      \disloc4{\mbox{def.\ by induction on $A$}}
                    }
                  } 
                }      
              }
            }
          }
        }
        \)
      }
      \column{\strut\\\disloc3{$t$ is a proof of $A$}}
    }
  }

  \dis3{Like typing, realising is a relation between terms and formulae}
}

\Slide[Example]{
  Consider a closed term $t$:
  \begin{tabular}{lll}
    $\vdash t\col A\arr B$ &if $t=\l x.t'$ with $x\col A\vdash t'\col B$
    & \disloc3{\begin{tabular}l
        have to consider terms\\[-5pt]
        with free variables
      \end{tabular}}\\
    & or $t=t_1\ t_2$ with
    \begin{tabular}l
      $t_1\col C\arr A\arr B$\\[-5pt]
      $t_2\col C$\\[-5pt]
      for some $C$
    \end{tabular}\\\\
    \disloc2{$t\Vdash A\arr B$} &
    \disloc2{%
      \begin{tabular}r
        if for all $t'$ such that $t'\Vdash A$,\\[-5pt]
        we have $t\ t'\Vdash B$
      \end{tabular}}&
    \disloc3{may consider closed terms only}
  \end{tabular}
}

\Slide[Why is this interesting?]{

  \dis1{Typing has been sold to you for safety:\\
    \flush\bord{``Well-typed programs cannot go wrong''} (Milner)\hfill\strut\\
    Hence the expression ``\baam{type-safety}''
  }

  \dis2{We could argue that in fact, we do not care about \rouge{typing}, but \bleu{realisability}:

    When implementing a function from natural numbers to natural numbers,\\
    we do not care whether our code $t$ satisfies \rouge{$t\col \texttt{int}\arr\texttt{int}$}\\
    \flush (in other words, whether $t=\l x.t'$ with\ldots or $t=t_1\ t_2$ with\ldots)
  }

  \dis3{But what we really care about is whether,\\
    when applying $t$ to an natural number, we compute a natural number.\\
    In other words, whether \bleu{$t\Vdash \texttt{int}\arr\texttt{int}$}
  }
}

\Slide[So, why did we ever do typing?]{

  \dis2{Well, because \bleu{realisability} is undecidable\\
    (given $t$ and $A$, determining whether \bleu{$t\Vdash A$})
  }

  \dis3{whereas \rouge{typing} is \disloc4{(usually)} decidable \disloc4{(with exceptions like Curry-style System F, etc)}\\
    (given $t$ and $A$, determining whether \rouge{$t\col A$})
  }

  \dis5{\baam{BUT} typing implies realising:
    \begin{center}
      if \bleu{$t\col A$} then \rouge{$t\Vdash A$}
    \end{center}
  }

  \dis6{It is the \baam{Adequacy Lemma}:\\
    typing is about syntax, realisability is about semantics\\
    \flush (writing \rouge{$t\Vdash A$} for \vert{$t\in \sem A{}$}, using notation of previous lectures)
  }

  \dis7{A slogan:
    \begin{center}
      \bord{Typing is a decidable approximation of realisability}
    \end{center}
  }

}


\Slide[Origins]{

  \dis1{Introduced by Kleene to formalise the Brouwer–Heyting–Kolmogorov interpretation of intuitionistic logic}

  \dis2{\[
    \begin{array}{ll}
      t\Vdash A_1\wedge A_2 &\mbox{if $t=\paire {t_1}{t_2}$ with $t_1\Vdash A_1$ and  $t_2\Vdash A_2$}\\
      t\Vdash A_1\vee A_2 &\mbox{if $t=\inj[i] {t'}$ with $t'\Vdash A_i$ for $i=0$ or $i=1$}\\
      t\Vdash A_1\arr A_2 &\mbox{if $t$ is a computable function such that, whenever $u\Vdash A_1$, $t(u)\Vdash A_2$}\\
      t\Vdash \exists x A(x)&\mbox{if $t=\paire {a}{t'}$ with $a$ an element of the ``model'' and $t'\Vdash A(a)$}\\
      t\Vdash \forall x A(x)&\mbox{if $t$ is a computable function such that,}\\[-5pt]
      &\mbox{for all elements $a$ of the ``model'', $t(a)\Vdash A(a)$}\\
    \end{array}
    \]}
  \dis3{Parameterised by a way to interpret atomic formulae}

  \dis4{$t$ ranges over mathematical objects such as pairs, computable functions, etc}
  \dis5{can be implemented as \bord{a number}\\
     \flush(ok for pairs, injections, \& computable functions can be assigned their Gödel numbers)}
  \dis6{can be implemented as an \bord{untyped $\lambda$-term} (untyped $\l$-calculus being Turing-complete)}
  \dis7{\flush \rouge{there comes Curry-Howard correspondence}}

}

\Slide[A few remarks]{

  \dis1{If \rouge{$t\col A$}, then Adequacy Lemma gives \bleu{$t\Vdash A$} \baam{for any} orthogonality relation $\bot$\\
    \flush (closed under anti-reduction)}
  \dis2{But typed $\lambda$-calculus is not Turing-complete:\\
    if we only use typed $\l$-terms as realisers, we are missing some computable functions, and hence some potential realisers!}
  \dis3{Also, think of how to \bleu{realise} $\forall x^{\mathbb N} A(x)$ and how to \rouge{prove} it:}
  \dis4{In order to \bleu{realise} $\forall x^{\mathbb N} A(x)$, we can, taking a natural number $n$ as input,\\
    give different realisers of $A(n)$ depending on $n$ (in any computable way)}
  \dis5{In order to \rouge{prove} $\forall x^{\mathbb N} A(x)$, we need to produce a single proof, of $A(x)$\\
    (\ie a generic way of proving $A(n)$, not depending on $n$)}

}

\Slide[And what about classical logic]{
  
  \dis1{Origins are really about constructivism:\\
    a \bleu{realiser} of $\exists x A(x)$ can only be a pair whose first component is a witness\\
    a \bleu{realiser} of $A_1\vee A_2$ can only be one of the 2 injections
  }

  \dis2{Doing something similar in classical logic seems difficult}

  \dis3{But, since Griffin's connection between control and classical proofs,\\
    realisability has received renewed attention, mostly by Krivine et al.
  }
}

\Slide[Where polarities and orthogonality come back]{
  \dis1{Idea:
    \begin{itemize}
    \item take an orthogonality relation $\bot$ between ``proofs'' and ``counter-proofs'' (\ie between things that could be realisers), closed under \rouge{anti-reduction}
    \item define a \baam{raw} interpretation of positive formulae as in intuitionistic logic
    \item define the interpretation of negative formulae as their \remph{orthogonals}
    \item define the interpretation of positive formulae as their \remph{bi-orthogonals}
    \end{itemize}
  }
  \dis2{
    \[\begin{array}{|ll|}
      \hline
      \SemTyr {A_1\vee A_2}\sigma&\eqdef\{\inj[i]t\mid t\in \SemTyr {A_i}\sigma\}\\
      \SemTyr {\exists x A}\sigma&\eqdef\{\paire{a}{t}\mid t\in\SemTyr A{\sigma,x\mapsto a}\}\\
      \SemTyr {N}\sigma&\eqdef\SemTy N\sigma\\
      \hline
      \SemTy N\sigma&\eqdef\uniorth{(\SemTyr{\uniorth N}\sigma)}\\
      \hline
      \SemTy P\sigma&\eqdef\biorth{(\SemTyr{P}\sigma)}\\
      \hline
    \end{array}
    \]
  }
  \dis3{By taking $t\Vdash A$ to mean $t\in\SemTy A{}$, \vert{\bf Adequacy} now works in classical logic too:}
  \dis4{If \rouge{$\vdash_c t\col A$} \gray{($t$ classical proof of $A$)}, then \baam{for any} $\bot$ \gray{(closed under anti-reduction)} \bleu{$t\Vdash A$}}
}

\Slide[Remarks]{
  \dis1{Syntax for $t$ deliberately left abstract, but can use Curien-Herbelin-Wadler's calculus\\
    \flush (see exercise sheet)}
  \dis2{Some properties lost:\\
    Because we have taken orthogonals,\\
    From $t\Vdash A_1\vee A_2$ we do not necessarily have $t$ of the form $\inj[i]{t'}$ with $t'\Vdash A_i$\\
    \disloc3{From $t\Vdash \exists x A(x)$ we do not necessarily have $t$ of the form $\paire a {t'}$ with $a$ witness and \ldots}
  }
  \dis4{Witness extraction fails in classical realisability (as expected)\ldots}
  \dis5{\ldots unless $A(x)$ is of a particular form!\flush (see exercise sheet)}
}

\Slide[Conclusion]{

  \dis1{Realisability is a semantical notion}
    \begin{itemize}
      \dis2{\item that is entailed by typing\vfill}
      \dis3{\item that can be adapted to classical logic,\\
        despite having been introduced for very constructivist motivations}
      \dis4{\item that nicely accounts for polarisation, orthogonality \rouge{and focusing}}
      \dis5{\item that allows to build models from other models to prove relative consistency theorems:\\
        To prove ``Theory A is consistent if Theory B is consistent'',\\
        it suffices to transform a given model of B into a model of A.\\
        Set theorists do this everyday with the notion of \rouge{forcing}: \bleu{$p\Vdash A$} ``p forces $A$''\\
        Krivine showed that realisability generalises forcing.\\
        With realisability, set theory axioms can be explained with computational notions\\
        \flush (control, clock, global state and memory management, \etc)
      }
    \end{itemize}

}


==> 4_LAF/Non-deterministic.tex <==
\section{Sequent calculus with non-deterministic naming}

\begin{definition}[Formulae]\strut

  Let $\varF$ be a set of elements called \Index{variables}, denoted $\alpha,\beta,\ldots$.

  \Index{Terms} $r,r',\ldots$ are elements of a self-substitutive $\varF$-nominal algebra $\Terms$.
  %% \[\begin{array}{ll}
  %% \left(\Terms,
  %%      {\footnotesize
  %%        \begin{array}{c@{}l@{}l}
  %%          \Terms\times\varF\times\Terms&\rightarrow&\Terms\\
  %%          (r_0,\alpha,r)&\mapsto&\subst {r_0} \alpha r
  %%        \end{array}
  %%      }
  %%      \right)
  %% \end{array}
  %% \]
  %% such that %$\non{\non l}=l$, $\non {(\subst l \alpha r)} = \subst {\non l} \alpha r$, and 
  %% $\subst{\subst {r_0} \alpha r}\beta s = \subst{\subst {r_0} \beta s}\alpha {\subst r \beta s}$.

  \Index{Literals} $l,l',\ldots$ are elements of a $\Terms$-substitutive $\varF$-nominal algebra $\Lit$.
  %% \[\begin{array}{ll}
  %% \left(\Lit,
  %%      {\footnotesize
  %%        %% \left(
  %%        %% \begin{array}{c@{}l@{}l}
  %%        %%   \Lit&\rightarrow&\Lit\\
  %%        %%   l&\mapsto&\non l
  %%        %% \end{array}
  %%        %% \right),
  %%        \begin{array}{c@{}l@{}l}
  %%          \Lit\times\varF\times\Terms&\rightarrow&\Lit\\
  %%          (l,\alpha,r)&\mapsto&\subst l \alpha r
  %%        \end{array}
  %%      }
  %%      \right)
  %% \end{array}
  %% \]
  %% such that %$\non{\non l}=l$, $\non {(\subst l \alpha r)} = \subst {\non l} \alpha r$, and 
  %% $\subst{\subst l \alpha r}\beta s = \subst{\subst l \beta s}\alpha {\subst r \beta s}$.

  \Index{Formulae} $A,B,\ldots$ are elements of a $\Terms$-substitutive $\varF$-nominal algebra $\Forms$.
  %% \[\begin{array}{ll}
  %% \left(\Forms,
  %%      {\footnotesize
  %%        %% \left(
  %%        %% \begin{array}{c@{}l@{}l}
  %%        %%   \Lit&\rightarrow&\Forms\\
  %%        %%   l&\mapsto&l
  %%        %% \end{array}
  %%        %% \right),
  %%        \begin{array}{c@{}l@{}l}
  %%          \Lit\times\varF\times\Terms&\rightarrow&\Lit\\
  %%          (l,\alpha,r)&\mapsto&\subst l \alpha r
  %%        \end{array}
  %%      }
  %%      \right)
  %% \end{array}
  %% \]
  %% such that %$\non{\non l}=l$, $\non {(\subst l \alpha r)} = \subst {\non l} \alpha r$, and 
  %% $\subst{\subst A \alpha r}\beta s = \subst{\subst A \beta s}\alpha {\subst r \beta s}$.
\end{definition}

\begin{definition}[Formulae decompositions]\strut

  \Index{Formulae decompositions} $\Delta,\Del',\ldots$ are elements of an algebra
  \[\begin{array}{ll}
  \left(\SubsType,
       {\footnotesize
         \left(\begin{array}{c@{}l@{}l}
           \Lit&\rightarrow&\SubsType\\
           l&\mapsto&l
         \end{array}\right),
         \left(\begin{array}{c@{}l@{}l}
           \Forms&\rightarrow&\SubsType\\
           A&\mapsto&A
         \end{array}\right),
         \left(\begin{array}{l}
           \SubsType\\
           \Dunit
         \end{array}\right),
         \left(\begin{array}{c@{}l@{}l}
           \SubsType^2&\rightarrow&\SubsType\\
           (\Delta_1,\Delta_2)&\mapsto&\Delta_1\Dand\Delta_2
         \end{array}\right),
         \left(\begin{array}{c@{}l@{}l}
           \varF\times\SubsType&\rightarrow&\SubsType\\
           (\alpha,\Delta)&\mapsto&\Dex\alpha\Delta
         \end{array}
         \right)
       }
       \right)
  \end{array}
  \]
\end{definition}

\begin{definition}[Typing Contexts]
  Let $\var^+$and $\var^-$ be two nominal sets, of elements called \Index{positive labels} and \Index{negative labels}, respectively.

  \Index{Typing Contexts} $\Gamma,\Gamma',\ldots$ are elements of a nominal algebra
  \[\begin{array}{ll}
    \left(\Contexts,
      {\footnotesize
        \left(\begin{array}{c@{}l@{}l}
            \Contexts\times\var^+&\Rightarrow&\Lit\\
            (\Gam,x^+)&\mapsto&\varRead[x^+]\Gam
          \end{array}\right),
        \left(\begin{array}{c@{}l@{}l}
            \Contexts\times\var^-&\Rightarrow&\mathcal F\\
            (\Gam,x^-)&\mapsto&\varRead[x^-]\Gam
          \end{array}\right),
        \left(\begin{array}{c@{}l@{}l}
            \Contexts\times\SubsType&\Rightarrow&\Contexts\\
            (\Gam,\Delta)&\mapsto&\Gam\Cextend\Delta
          \end{array}\right)
      }
    \right)
  \end{array}
  \]
\end{definition}

\begin{definition}[Proof-Terms]
  Let \(\Data\) be a set of elements called \Index{patterns}.

  Proof-terms are defined by the following syntax:
  \[
  \begin{array}{lll@{\recdef}l}
    \mbox{Positive terms }&\PTerms^+&t^+&p\sigma\\
%    \mbox{Negative terms }&\PTerms^-&t^-&x^- \mid f\\
    \mbox{Substitutions }&\Subs&\sigma&\Tunit\mid\sigma_1\Tand\sigma_2 \mid \Tex r \sigma \mid x^+ \mid \THO f\\
    \mbox{Commands}&\PTerms&c& \cutc{x^-}{t^+} \mid \cutc{f}{t^+}
  \end{array}
  \]
  where $p$ ranges over patterns, $x^+$ ranges over $\var^+$, $x^-$ ranges over $\var^-$, $x$ ranges over $\NamingConvs$ and $f$ ranges over $\Data\rightarrow\PTerms$.
\end{definition}


\begin{definition}[\LKF]
  Assume we are given
  \begin{itemize}
  \item a equivariant relation $(\DerDec{}{\_}{\XcolY \_{\_}}):(\SubsType\times\Data\times\Forms)$
  \end{itemize}

  We define in Fig.~\ref{def:LKTh} the derivability of three typing judgements
  \begin{itemize}
  \item $(\DerF\_ {\XcolY {\_} \_}{})\quad:\quad(\Contexts\times \PTerms^+\times\Forms)$
  \item $(\Der\_ {\XcolY \_ \_})\quad:\quad(\Contexts\times \Subs\times\SubsType)$
  \item $(\Der\_ \_)\quad:\quad(\Contexts\times \PTerms)$
  \end{itemize}

\end{definition}


\begin{figure}[h]
  \[
  \begin{array}{|c|}
    \upline\\
    \infer[\textsf{sync}]
    {\DerF\Gam {\XcolY {p\sigma} A}{}}
    {\DerDec{}{\Delta}{\XcolY p{A}}
      \quad\Der{\Gamma}{\XcolY \sigma{\Delta}}}
    \\
    \midline
    \\
    \infer{\Der\Gam{\XcolY{\Tunit}{\Dunit}}}{\strut}
    \qquad
    \infer{\Der\Gam{\XcolY{\sigma_1\Tand\sigma_2}{\Del_1\Dand\Del_2}}}
    {\Der\Gam{\XcolY{\sigma_1}{\Del_1}}
      \quad
      \Der\Gam{\XcolY{\sigma_2}{\Del_2}}}
    \qquad
    \infer{\Der\Gam{\XcolY{\Tex r\sigma}{\Dex\alpha {\Del}}}}
    {\Der\Gam{\XcolY{\sigma}{\subst{\Del}\alpha r}}}
    \\\\
    \infer%[{[l\in\mathcal P]}]
    {\Der{\Gam}{\XcolY{x^+}{l}}}{\getvar[x^+]\Gam l}
    \qquad
    \infer[\textsf{async}]
    {\Der\Gam {\XcolY {\THO f} A}}
    {\forall \fresh p f,\forall\fresh\Delta\Gamma,\quad
      \DerDec{}{\Delta}{\XcolY p{A}}\quad\imp\quad\Der{\Gamma\Cextend[x]\Delta}{f(p)}}
    \\
    \midline
    \\
    \infer[\textsf{select}]{\Der\Gam{\cutc{x^-}{t^+}}}
    {\getvar[x^-]\Gam {A}\quad\DerF\Gam {\XcolY{t^+}A} {}}
    \qquad
    \infer[\cut]{\Der\Gam{\cutc{f}{t^+}}}
    {\Der\Gam {\XcolY {f}{A}}\qquad
      \DerF\Gam {\XcolY{t^+}A} {}}
    \\\downline
  \end{array}
  \]
\caption{\LKF}
\label{def:LKF}
\end{figure}

\begin{lemma}[Equivariance of typing]
The judgements derived by the rules of Fig.~\ref{def:LKF} are equivariant:
  \begin{itemize}
  \item $(\DerF\_ {\XcolY {\_} \_}{})\quad:\quad(\Contexts\times \PTerms^+\times\Forms)$
  \item $(\Der\_ {\XcolY \_ \_})\quad:\quad(\Contexts\times \Subs\times\SubsType)$
  \item $(\Der\_ \_)\quad:\quad(\Contexts\times \PTerms)$
  \end{itemize}
\end{lemma}


==> 8_DPLL/Conclusion.tex <==
\section {Conclusion and Further work}
\label{sec:DPLLconc}

In this chapter we have identified an elementary \DPLLTh\ procedure
and established a bisimulation with the gradual construction of
proof-trees in \LKThp\ according to a simple strategy.

While \LKThp\ differs from the inference system of~\eg
\cite{Tin-JELIA-02} (\eg we still take formulae to be trees and
inference rules to organise the root-first decomposition of their
connectives, rather than using \DPLLTh's more flexible structures), it
would be interesting to capture some of the related systems that
extend \DPLLTh\ with \eg full first-order logic and/or
equality~\cite{Baumgartner00,BaumgartnerT08,BaumgartnerT11}.  The full
version of \LKThp\ is indeed designed for handling quantifiers and
equalities, so we hope to relate it to other techniques such as
unification, paramodulation, superposition, etc.

This is also our challenge for the \Psyche\ implementation: ideally,
try to show how the smart mechanisms that we know to be efficient at
proving something, can be emulated or decomposed into an interaction
between our kernel and a specific plugin to be programmed. This would
turn \Psyche\ into a modular and collaborative platform, a standard
format of problem-solving mechanisms where each technique can play its
part, be it from start to finish, or in collaboration with each other
or a human user.

We can imagine using a proof assistant to prove \Psyche's
correctness~\cite{chargueraud-10-cfml}, since the kernel is small, not
using any imperative features, and the plugins need not be
certified. This approach is an alternative to existing techniques of
certification of SMT tools (or of any other technique that could
instead be implemented as a \Psyche\ plugin).
%with formal proofs of automated decision procedures such as SMT tools.  
%% Moreover the certification of the possible extensions of the kernel to
%% more expressive logics is far more incremental than the
%% re-implementations, in a proof assistant, of their associated formal
%% proof-producing decision procedures.

% Also in a proof assistant like Coq which retains proof objects, the size of the formal proofs would be dramatically smaller. In the current approaches, it depends on the often huge size of the trace output by the automated prover (e.g. the SMT tool). In the case we propose, it is only the size of the proof of the kernel (plus the ones of the theory lemmas).


==> Macros/old/Macros_0Basics.tex <==
%Relations

\newcommand\red{\rightarrow}

\newcommand\pfunspace{\rightharpoonup}

\newcommand\inve[1]{{#1}^{-1}}
\newcommand\co[2]{{#1}\cdot{#2}}
\newcommand\Id[1][]{\textsf{Id}_{#1}}
\newcommand\suc[2]{\hspace{0.1cm}#1\hspace{-0.1cm}(#2)}
\newcommand\induced[2]{{#1}[#2]}

\newcommand\restr[2]{{#1}_{|#2}}

%Normalisation
\newcommand\patriarchal{patriarchal}
\newcommand\paternal{paternal}

\newcommand\rf[1]{\textsf{rf}^{#1}}
\newcommand\nf[1]{\textsf{nf}^{#1}}
\newcommand\SN[1]{\textsf{SN}^{#1}}
\newcommand\BN[2]{\textsf{BN}^{#1}_{#2}}
\newcommand\WN[1]{\textsf{WN}^{{#1}}}

\newcommand\RM[1]{\mathcal M_{#1}}
\newcommand\Remul{\mathcal W}
\newcommand{\multiset}[1]{\{ \!\! \{ #1\} \!\! \} }

\newcommand\lex{{\textsf{lex}}}
\newcommand\mul{{\textsf{mul}}}
\newcommand\lexx{{\textsf{lexx}}}
\newcommand\mull{{\textsf{mull}}}


%RPO=========================================

\newcommand{\llex}[1][<]{{#1}_{\lex}}
\newcommand{\glex}[1][>]{{#1}_{\lex}}

\newcommand{\lmul}[1][<]{{#1}_{\mul}}
\newcommand{\gmul}[1][>]{{#1}_{\mul}}

\newcommand{\lllex}[1][<]{{#1}_{\lexx}}
\newcommand{\gllex}[1][>]{{#1}_{\lexx}}

\newcommand{\lmull}[1][<]{{#1}_{\mull}}
\newcommand{\gmull}[1][>]{{#1}_{\mull}}

\newcommand\RPO{{\textsf{RPO}}}
\newcommand\LPO{{\textsf{LPO}}}
\newcommand\MPO{{\textsf{MPO}}}

\newcommand{\grpo}{\mbox{$>\!\!>$}}
\newcommand{\lrpo}{\mbox{$<\!\!<$}}

\newcommand{\glpo}{\mbox{$>\!\!>$}}
\newcommand{\llpo}{\mbox{$<\!\!<$}}

\newcommand{\gmpo}{\mbox{$>\!\!>$}}
\newcommand{\lmpo}{\mbox{$<\!\!<$}}

\ignore{
\newcommand{\grpo}[1][>]{{{#1}_{\textsf{rpo}}}}
\newcommand{\lrpo}[1][<]{{{#1}_{\textsf{rpo}}}}

\newcommand{\glpo}[1][>]{{{#1}_{\textsf{lpo}}}}
\newcommand{\llpo}[1][<]{{{#1}_{\textsf{lpo}}}}

\newcommand{\gmpo}[1][>]{{{#1}_{\textsf{mpo}}}}
\newcommand{\lmpo}[1][<]{{{#1}_{\textsf{mpo}}}}
}

\newcommand\pre{\prec}


%1st-order syntax======================================

\newcommand{\blob}{\star}
\newcommand\blobx[1]{\textsf{c}^{#1}}

\newcommand\uni[2]{\textsf{uni}(#1)}
\newcommand\bi[2]{\textsf{ii}(#1,#2)}

\newcommand\un[1]{\textsf{i}(#1)}
\newcommand\deux[2]{\textsf{ii}(#1,#2)}
\newcommand\two[2]{{\textsf{II}(#1,#2)}}

\newcommand\folet[2]{\textsf{let}(#1,#2)}
\newcommand\foap[2]{\textsf{ap}(#1,#2)}


\newcommand\varl[1]{\textsf{par}(#1)}
\newcommand\vart[2]{\textsf{cut}(#1,#2)}
\newcommand\coup[3][{}]{{\textsf{cut}}^{#1}(#2,#3)}
\newcommand\subf[3][{}]{\textsf{sub}^{#1}(#2,#3)}
\newcommand\subfc[2]{\textsf{subc}(#1,#2)}

\newcommand\focut[3][{}]{{\textsf{cut}^{#1}(#2,#3)}}
\newcommand\fosub[3][{}]{{\textsf{sub}^{#1}(#2,#3)}}

\newcommand\foP[3]{\deux {#2}{#3}}
\newcommand\folami[3]{\deux {#2}{#3}}
\newcommand\focontv[2]{\un{#2}}
\newcommand\focont[3][{}]{\focut[#1]{#2}{#3}}

\newcommand\foel{\blob}
\newcommand\foconc[2]{\deux {#1}{#2}}
\newcommand\fost[2]{\deux {#1}{#2}}

\newcommand\focuti[5][{}]{\fosub[#1]{#3}{#5}}


==> Macros/old/Macros_0HOC.tex <==
%SYNTACTIC CATEGORIES
\newcommand\HOC{{\textsf{HOC}}}
\newcommand\HRS{{\textsf{HRS}}}
\newcommand\CRS{{\textsf{CRS}}}
\newcommand\ERS{{\textsf{ERS}}}
\newcommand\SERS{{\textsf{SERS}}}
\newcommand\IS{{\textsf{IS}}}
\newcommand\BNF{{\textsf{BNF}}}


\newcommand\SC{\mathcal{SC}}
\newcommand\SCmeta{\mathcal{SC}^{\mathcal M}}
\newcommand\HOSC[1]{\textsf{HOSC}_{#1}}

\newcommand{\sep}{\mbox{\bf\;|\;}}    % Separators in BNF definitions
\newcommand\mT{_{\mathcal T}}


\newcommand\arrsc{\hookrightarrow}
\newcommand{\colsc}{\wr}
\newcommand{\tsc}[2]{{#1}\colsc{#2}}

\newcommand{\order}[1]{\textsf{order}(#1)}
\newcommand{\arity}[1]{\textsf{arity}(#1)}

%TERMS

%\newcommand\sensible{sensible}

\newcommand\subterm{\sqsubset}
\newcommand\subtermeq{\sqsubseteq}
\newcommand\susterm{\sqsupset}
\newcommand\sustermeq{\sqsupseteq}
\newcommand\sizeof[1]{\textsf{s}({#1})}
\newcommand\height[2]{\textsf{h}_{#1}({#2})}

\newcommand{\se}{\equiv}

\newcommand{\cc}[1]{\textbf{cc}{#1}}

\newcommand\FV[2][{}]{\textsf{FV}_{#1}(#2)}
\newcommand\FVname{\textsf{FV}}
\newcommand\doma[1]{\textsf{Support}(#1)}
\newcommand\domaname{\textsf{Support}}

\newcommand\alphaeq{=_\a}
\newcommand\aeq[3]{{#1}\vdash {#2}=_\a{#3}}
\newcommand\vrel[2]{{#1}-{#2}}
\newcommand\aeqv[3]{{#1}\vdash \vrel {#2}{#3}}

%META
\newcommand\mX{\mathbb{X}}
\newcommand\mY{\mathbb{Y}}
\newcommand\mM{\mathbb{M}}
\newcommand\mN{\mathbb{N}}
\newcommand\mE{\mathbb{E}}
\newcommand\mS{\mathbb{S}}
\newcommand\mB{\mathbb{B}}
\newcommand\mA{\mathbb{A}}
\newcommand\mP{\mathbb{P}}
\newcommand\mUU{\mathbb{U}}
\newcommand\mTT{\mathbb{T}}
\newcommand\mVar[1][{}]{\textsf{V}_{#1}}
\newcommand\Lists[1][{}]{\textsf{Lists}_{#1}}
\newcommand\Multisets[1][{}]{\textsf{Multisets}_{#1}}
\newcommand\Sets[1][{}]{\textsf{Sets}_{#1}}

\newcommand\metaC[1]{{#1}^\dagger}
\newcommand\metaCname{{}^\dagger}

\newcommand\arrmeta{\times}
\newcommand\arrm{\rightharpoonup}
\newcommand{\colscm}{\ \vdots\ }
\newcommand{\tscm}[2]{{#1}\colscm{#2}}


\newcommand\BV[2]{\textsf{AVe}_{#1}(#2)}
\newcommand\BVm[2]{\textsf{AVs}_{#1}(#2)}
\newcommand\FMV[1]{\textsf{MV}(#1)}
\newcommand\BConv[1]{\textsf{SC}(#1)}

\newcommand\SetT{\mathcal {S}\textsf{et}}

\newcommand\toHRS[2]{\theta_{#1} {(#2)}}
\newcommand\toHRSname{\theta }
\newcommand\etalf[2][{}]{\eta_{#1}{(#2)}}

%REWRITE

\newcommand{\subst}[3]{ \left\{{}^{#3}\hspace{-.2em}\diagup\hspace{-.2em}_{#2} \right\} #1 }
\newcommand{\Ren}[3]{\subst {#1} {#2} {#3}}
\newcommand{\Rene}[3]{\subst {#1} {\_} {#3}}


%\newcommand{\Ren}[3]{\mathcal{R}_{#3}^{#2}({#1})}
%\newcommand{\Rene}[3]{\mathcal{R}_{#3}({#1})}
%\newcommand{\esubst}[2]{[#1/#2]}

\newcommand{\ren}[3]{({#1}\;{#2}) {#3}}
\newcommand{\renyx}[1]{\ren{y}{x}{#1}}

\renewcommand{\root}{\textsf{\tiny{r\,o\,o\,t}}}
\newcommand{\Rew}[2][]{\stackrel{#1}{\longrightarrow}_{#2}\;}
\newcommand{\Rewn}[2][*]{{\longrightarrow}^{#1}_{#2}\;}
\newcommand{\Rewplus}[2][+]{{\longrightarrow}^{#1}_{#2}\;}
\newcommand{\Rewsn}[2][*]{{\longleftrightarrow}^{#1}_{#2}\;}



==> Macros/old/Macros_10Fomega.tex <==

%Derivability

\newcommand\DerFomT[3]{\Deri[\FomegaC]{#1}{#2}{#3}}
\newcommand\DerFomTs[4]{\Deris[\FomegaC]{#1}{#2}{#3}{#4}}
\newcommand\Derwf[2]{\textsf{wf}_{#1}(#2)}
\newcommand\DerFomt[4]{\Derif[\FomegaC]{#1}{#2}{#3}{#4}}
\newcommand\DerFomp[3]{\Derif[\FomegaC]{#1}{#2}{#3}\diamond}

%Syntax
%Kinds

\newcommand\Arr[2]{{#1}\rightarrow {#2}}

%Types
\newcommand\andP{{\wedge^+}}
\newcommand\andN{{\wedge^-}}
\newcommand\orP{{\vee^+}}
\newcommand\orN{{\vee^-}}
\newcommand\imp{\Rightarrow}

\newcommand\EX[3][]{\exists #2^{#1} #3}
\newcommand\FA[3][]{\forall #2^{#1} #3}

\newcommand{\non}[1]{{#1}^{\perp}}
\newcommand{\eqT}{\approx}


\newcommand{\varT}{\textsf{Var}^T}
\newcommand{\fall}[3][{}]{\forall{#2}^{#1}.{#3}}
\newcommand{\xists}[3][{}]{\exists{#2}^{#1}.{#3}}
\newcommand{\et}[2]{{#1}\wedge {#2}}
\newcommand{\ou}[2]{{#1}\vee {#2}}
%\newcommand{\impl}[2]{{#1}\arr {#2}}
\newcommand{\nega}[1]{\overline{#1}}
\newcommand{\lamb}[3]{\lambda{#2}^{#1}.{#3}}
\newcommand{\dual}[1]{{#1}^{\bot}}
\newcommand{\bidual}[1]{{#1}^{\bot\bot}}
\newcommand{\tridual}[1]{{#1}^{\bot\bot\bot}}

\newcommand\ex [3][]{{#2}^{#1}.#3}
%\newcommand\exT[3][]{{#2}^{#1}.#3}

\newcommand\xistscod[3][{}]{\exists^{\textsf{cod}}{#2}^{#1}.{#3}}
\newcommand{\etcod}[2]{{#1}\wedge^{\textsf{cod}} {#2}}
\newcommand{\oucod}[2]{{#1}\vee^{\textsf{cod}} {#2}}

% %\newcommand\andP{\otimes}
% %\newcommand\andN{\&}
% %\newcommand\orP{\oplus}
% %\newcommand\orN{\vee^-}
% %\newcommand\imp{\multimap}

%Terms
\newcommand\proji[2]{#1}
\newcommand\projii[2]{#2}





% Sets
\newcommand{\var}{\textsf{Var}}
\newcommand{\varF}[1][]{\textsf{Var}^{#1}}

\newcommand{\Lit}{\mathcal L}
\newcommand{\Terms}[1][]{\mathcal R^{#1}}
\newcommand{\Forms}{\mathcal F}
\newcommand{\Just}{\mathcal J}
\newcommand{\Data}{\mathcal P}
\newcommand{\PTerms}{\mathcal H}
\newcommand{\Subs}{\mathcal S}
\newcommand{\SubsType}{\mathcal D}
\newcommand{\Contexts}{\mathcal G}

% Substitutions
\newcommand\Tand{,}
\newcommand\Tunit{\bullet}
\newcommand\Tex[3][]{{#2}^{#1}.{#3}}

% SubstitutionsTypes
\newcommand\Dand{,}
\newcommand\Dunit{\bullet}
\newcommand\Dex[3][]{{#2}^{#1}.{#3}}

% Contexts
\newcommand\Cextend{;}



%\newcommand{\lamc}[4][{}{}]{{#2}^{\i #1}{#3}^{\ii #1}.{#4}}
%\newcommand\stac[2]{{#1}\cdot{{#2}}}
\newcommand{\inj}[4][{}{}]{\lambda #2^{\proji #1}#3^{\projii #1}.{#4}}
\newcommand\paire[2]{\langle{#1},{#2}\rangle}
%\newcommand{\switch}[1]{\bullet #1}

\newcommand{\Lamb}[3]{\Lambda{#2}^{#1}.{#3}}
\newcommand{\appl}[2]{\langle #1,#2\rangle}

\newcommand\cutc[2]{\{#1\bullet#2\}}
\newcommand\just[1]{\{#1\}}
\newcommand\down[1]{\downarrow\!#1}


\newcommand{\m}[3][{}]{\mu #2^{#1}\!.{#3}}
%\newcommand{\mt}[3][{}]{\tilde\mu {#2}^{#1}.{#3}}



%Semantics:

\newcommand{\semK}[1]{[\![#1]\!]}
\newcommand{\swapK}[2]{\textsf{swap}_{#1}{#2}}

\newcommand{\sem}[2]{[\![#2]\!]_{#1}}
\newcommand{\semt}[1]{[\![#1]\!]}
% \newcommand\sem[2]{[#1]_{#2}}

\newcommand{\orth}[2]{{#1\mathrel{{\perp}}#2}}

\newcommand{\effac}[1]{\|{#1}\|}
\newcommand{\twt}{\mathcal{T}}

\newcommand{\mU}{\mathcal U}
\newcommand{\mV}{\mathcal V}

\newcommand{\fp}[2]{\Phi_{#1}{#2}}
\newcommand\LamC[1]{\Lambda\_.{#1}}
\newcommand\applC[1]{\appl{\_}{#1}}

%======================
%Relationship with other formalisms

%Derivability in Fomega normal

\newcommand\DerFomiT[3]{\Deri[\Fomega]{#1}{#2}{#3}}
\newcommand\DerFomitwf[2]{\textsf{wf}^{#1}_{\Fomega}(#2)}
\newcommand\DerFomit[4]{\Derif[\Fomega]{#1}{#2}{#3}{#4}}

\newcommand\SNC{\SN{\B'\x'}_{\textsf{TC}}}
\newcommand\SNl{\SN{\B'\x'}_{\textsf{TL}}}


==> Macros/old/Macros_1Basics.tex <==
%Relations

\newcommand\red{\rightarrow}

\newcommand\inve[1]{{#1}^{-1}}
\newcommand\co[2]{{#1}\cdot{#2}}
\newcommand\Id[1][]{\textsf{Id}_{#1}}
\newcommand\suc[2]{\hspace{0.1cm}#1\hspace{-0.1cm}(#2)}
\newcommand\induced[2]{{#1}[#2]}

\newcommand\restr[2]{{#1}_{|#2}}

%Normalisation
\newcommand\patriarchal{patriarchal}
\newcommand\paternal{paternal}

\newcommand\rf[1]{\textsf{rf}^{#1}}
\newcommand\nf[1]{\textsf{nf}^{#1}}
\newcommand\SN[1]{\textsf{SN}^{#1}}
\newcommand\BN[2]{\textsf{BN}^{#1}_{#2}}
\newcommand\WN[1]{\textsf{WN}^{{#1}}}

\newcommand\RM[1]{\mathcal M_{#1}}
\newcommand\Remul{\mathcal W}
\newcommand{\multiset}[1]{\{ \!\! \{ #1\} \!\! \} }

\newcommand\lex{{\textsf{lex}}}
\newcommand\mul{{\textsf{mul}}}
\newcommand\lexx{{\textsf{lexx}}}
\newcommand\mull{{\textsf{mull}}}


%RPO=========================================

\newcommand{\llex}[1][<]{{#1}_{\lex}}
\newcommand{\glex}[1][>]{{#1}_{\lex}}

\newcommand{\lmul}[1][<]{{#1}_{\mul}}
\newcommand{\gmul}[1][>]{{#1}_{\mul}}

\newcommand{\lllex}[1][<]{{#1}_{\lexx}}
\newcommand{\gllex}[1][>]{{#1}_{\lexx}}

\newcommand{\lmull}[1][<]{{#1}_{\mull}}
\newcommand{\gmull}[1][>]{{#1}_{\mull}}

\newcommand\RPO{{\textsf{RPO}}}
\newcommand\LPO{{\textsf{LPO}}}
\newcommand\MPO{{\textsf{MPO}}}

\newcommand{\grpo}{\mbox{$>\!\!>$}}
\newcommand{\lrpo}{\mbox{$<\!\!<$}}

\newcommand{\glpo}{\mbox{$>\!\!>$}}
\newcommand{\llpo}{\mbox{$<\!\!<$}}

\newcommand{\gmpo}{\mbox{$>\!\!>$}}
\newcommand{\lmpo}{\mbox{$<\!\!<$}}

\ignore{
\newcommand{\grpo}[1][>]{{{#1}_{\textsf{rpo}}}}
\newcommand{\lrpo}[1][<]{{{#1}_{\textsf{rpo}}}}

\newcommand{\glpo}[1][>]{{{#1}_{\textsf{lpo}}}}
\newcommand{\llpo}[1][<]{{{#1}_{\textsf{lpo}}}}

\newcommand{\gmpo}[1][>]{{{#1}_{\textsf{mpo}}}}
\newcommand{\lmpo}[1][<]{{{#1}_{\textsf{mpo}}}}
}

\newcommand\pre{\prec}


%1st-order syntax======================================

\newcommand{\blob}{\star}
\newcommand\blobx[1]{\textsf{c}^{#1}}

\newcommand\uni[2]{\textsf{uni}(#1)}
\newcommand\bi[2]{\textsf{ii}(#1,#2)}

\newcommand\un[1]{\textsf{i}(#1)}
\newcommand\deux[2]{\textsf{ii}(#1,#2)}
\newcommand\two[2]{{\textsf{II}(#1,#2)}}

\newcommand\folet[2]{\textsf{let}(#1,#2)}
\newcommand\foap[2]{\textsf{ap}(#1,#2)}


\newcommand\varl[1]{\textsf{par}(#1)}
\newcommand\vart[2]{\textsf{cut}(#1,#2)}
\newcommand\coup[3][{}]{{\textsf{cut}}^{#1}(#2,#3)}
\newcommand\subf[3][{}]{\textsf{sub}^{#1}(#2,#3)}
\newcommand\subfc[2]{\textsf{subc}(#1,#2)}

\newcommand\focut[3][{}]{{\textsf{cut}^{#1}(#2,#3)}}
\newcommand\fosub[3][{}]{{\textsf{sub}^{#1}(#2,#3)}}

\newcommand\foP[3]{\deux {#2}{#3}}
\newcommand\folami[3]{\deux {#2}{#3}}
\newcommand\focontv[2]{\un{#2}}
\newcommand\focont[3][{}]{\focut[#1]{#2}{#3}}

\newcommand\foel{\blob}
\newcommand\foconc[2]{\deux {#1}{#2}}
\newcommand\fost[2]{\deux {#1}{#2}}

\newcommand\focuti[5][{}]{\fosub[#1]{#3}{#5}}

==> Macros/old/Macros_1Deriv.tex <==
%DERIVABILITY

% Types and Typing
\newcommand\arr{\hspace{-3pt}\rightarrow\hspace{-3pt}}
\newcommand\rto{\arr}
\renewcommand\>{\arr}

\newcommand\col{\unskip{\colon}}
\newcommand\XcolY[2]{#1\col#2}
\newcommand\varRead[2][]{#2_{|#1}}
\newcommand\getvar[3][]{#2_{|#1}=#3}


% Generic derivability symbol
\newcommand{\seqg}[3]{\mbox{$\ {#1}_{#2}^{#3}\ $}}

% ... with vdash and models and their negations
\newcommand{\seqf} [2][]{\seqg{\vdash}     {#1}{#2}}
\newcommand{\nseqf}[2][]{\seqg{\not\vdash} {#1}{#2}}
\newcommand{\satf} [2][]{\seqg{\models}    {#1}{#2}}
\newcommand{\nsatf}[2][]{\seqg{\not\models}{#1}{#2}}
\newcommand{\decf} [2][]{\seqg{\Vdash}    {#1}{#2}}
\newcommand{\ndecf}[2][]{\seqg{\not\Vdash}{#1}{#2}}
\newcommand{\decs} [2][]{\seqg{\Vvdash}    {#1}{#2}}
\newcommand{\ndecs}[2][]{\seqg{\not\Vvdash}{#1}{#2}}

%Purely logical

\newcommand\DerF[4][]{{#2}\seqf[{#1}]{}{[#3]}{#4}}
\newcommand\Der[3][]{{#2}\seqf[{#1}]{}{#3}}

\newcommand\Ders[3][]{{#2}\decs[{#1}]{}{#3}}

\newcommand\DertF[5][]{{#3}\seqf[{#1}]{#2}{[#4]}{#5}}
\newcommand\Dert[4][]{{#3}\seqf[{#1}]{#2}{#4}}

\newcommand\DerDec[4][]{{#3}\decf[{#1}]{#2}{#4}}

\newcommand\DerTF[4][]{{#2}\satf[{#1}]{}{[#3]}{#4}}
\newcommand\DerT[3][]{{#2}\satf[{#1}]{}{#3}}

%Per systems

\newcommand\DerDPLL[2] {{#1}\mbox{;}{#2}\seq}
\newcommand\DerFLKF[3][]{\seqf[{#1}]{} #2\Downarrow #3}
\newcommand\DerLKF[3][]{\seqf[{#1}]{}#2\Uparrow #3}
\newcommand\DerFlLJF[4][]{[#2]\stackrel{#3}{\longrightarrow}[#4]}
\newcommand\DerFrLJF[3][]{[#2]{-}_{#3}{\rightarrow}}
\newcommand\DerLJrF[4][]{[#2]#3\longrightarrow #4}
\newcommand\DerLJF[4][]{[#2]#3\longrightarrow [#4]}


%Rules

\newcommand\ax{\textsf{ax}}
\newcommand\cut{\textsf{cut}}
\newcommand\re{\hspace{4pt}\arr_{\textsf{elim}}}

\newcommand\weakening{\textsf{weak}}
\newcommand\contraction{\textsf{cont}}


%Proof-term Syntax

\newcommand\daggerL{\raise3pt\hbox{\rotatebox{-40}{$\dagger$}}}
\newcommand\daggerR{\raise0pt\hbox{\rotatebox{40}{$\dagger$}}}


\newcommand\letin[3]{\left\langle{#1}\dagger {#2}.{#3}\right\rangle}
\newcommand\ltin[1]{\{#1\}}
\newcommand\hole{[]}


% new for DPLL
%\newcommand{\seqgD}[4]{\mbox{$\ {#1}_{#2}^{#3}_(#4)\ $}}
%\newcommand{\seqfD}[2][]{\seqgD{\vdash}{#1}{#2}}
%end

%new for Theory
%\newcommand{\seqTh}[2][]{\seqg{\vdash_{\mathcal{T}}}{#1}{#2}}
%\newcommand{\seqThD}[2][]{\seqg{\vdash_{\mathcal{T}}^{\Delta_0}}{#1}{#2}} % for DPLL (for \Del_0)
% \newcommand{\seqThD}[2][]{\seqf[#1]\mathcal{T}}^{\mathcal P}}{#1}{#2}} % for DPLL \mathcal{P}
% \newcommand{\seqFOL}[2][]{\seqg{\vdash_{FOL}}{#1}{#2}} % First order Logic
% % end
% %new for Th
% \newcommand{\seqt}[1][]{\seqTh[#1]{}}
% \newcommand{\seqtD}[1][]{\seqThD[#1]{}}
% \newcommand{\seqFol}[1][]{\seqFOL[#1]{}}  %new for FOL
% %end


==> Macros/old/Macros_1HOC.tex <==
%SYNTACTIC CATEGORIES
\newcommand\HOC{{\textsf{HOC}}}
\newcommand\HRS{{\textsf{HRS}}}
\newcommand\CRS{{\textsf{CRS}}}
\newcommand\ERS{{\textsf{ERS}}}
\newcommand\SERS{{\textsf{SERS}}}
\newcommand\IS{{\textsf{IS}}}
\newcommand\BNF{{\textsf{BNF}}}


\newcommand\SC{\mathcal{SC}}
\newcommand\SCmeta{\mathcal{SC}^{\mathcal M}}
\newcommand\HOSC[1]{\textsf{HOSC}_{#1}}

\newcommand{\sep}{\mbox{$\;|\;$}}    % Separators in BNF definitions
\newcommand\mT{_{\mathcal T}}


\newcommand\arrsc{\hookrightarrow}
\newcommand{\colsc}{\wr}
\newcommand{\tsc}[2]{{#1}\colsc{#2}}

\newcommand{\order}[1]{\textsf{order}(#1)}
\newcommand{\arity}[1]{\textsf{arity}(#1)}

%TERMS

%\newcommand\sensible{sensible}

\newcommand\subterm{\sqsubset}
\newcommand\subtermeq{\sqsubseteq}
\newcommand\susterm{\sqsupset}
\newcommand\sustermeq{\sqsupseteq}
\newcommand\sizeof[1]{\textsf{s}({#1})}
\newcommand\height[2]{\textsf{h}_{#1}({#2})}

\newcommand{\se}{\equiv}

\newcommand{\cc}[1]{\textbf{cc}{#1}}

\newcommand\FV[2][{}]{\textsf{FV}_{#1}(#2)}
\newcommand\FVname{\textsf{FV}}
\newcommand\doma[1]{\textsf{Support}(#1)}
\newcommand\domaname{\textsf{Support}}

\newcommand\alphaeq{=_\a}
\newcommand\aeq[3]{{#1}\vdash {#2}=_\a{#3}}
\newcommand\vrel[2]{{#1}-{#2}}
\newcommand\aeqv[3]{{#1}\vdash \vrel {#2}{#3}}

%META
\newcommand\mX{\mathbb{X}}
\newcommand\mY{\mathbb{Y}}
\newcommand\mM{\mathbb{M}}
\newcommand\mN{\mathbb{N}}
\newcommand\mE{\mathbb{E}}
\newcommand\mS{\mathbb{S}}
\newcommand\mB{\mathbb{B}}
\newcommand\mA{\mathbb{A}}
\newcommand\mP{\mathbb{P}}
\newcommand\mUU{\mathbb{U}}
\newcommand\mTT{\mathbb{T}}
\newcommand\mVar[1][{}]{\textsf{V}_{#1}}
\newcommand\Lists[1][{}]{\textsf{Lists}_{#1}}
\newcommand\Multisets[1][{}]{\textsf{Multisets}_{#1}}
\newcommand\Sets[1][{}]{\textsf{Sets}_{#1}}

\newcommand\metaC[1]{{#1}^\dagger}
\newcommand\metaCname{{}^\dagger}

\newcommand\arrmeta{\times}
\newcommand\arrm{\rightharpoonup}
\newcommand{\colscm}{\ \vdots\ }
\newcommand{\tscm}[2]{{#1}\colscm{#2}}


\newcommand\BV[2]{\textsf{AVe}_{#1}(#2)}
\newcommand\BVm[2]{\textsf{AVs}_{#1}(#2)}
\newcommand\FMV[1]{\textsf{MV}(#1)}
\newcommand\BConv[1]{\textsf{SC}(#1)}

\newcommand\SetT{\mathcal {S}\textsf{et}}

\newcommand\toHRS[2]{\theta_{#1} {(#2)}}
\newcommand\toHRSname{\theta }
\newcommand\etalf[2][{}]{\eta_{#1}{(#2)}}

%REWRITE

\newcommand{\subst}[3]{ \left\{{}^{#3}\hspace{-.2em}\diagup\hspace{-.2em}_{#2} \right\} #1 }
\newcommand{\Ren}[3]{\subst {#1} {#2} {#3}}
\newcommand{\Rene}[3]{\subst {#1} {\_} {#3}}


%\newcommand{\Ren}[3]{\mathcal{R}_{#3}^{#2}({#1})}
%\newcommand{\Rene}[3]{\mathcal{R}_{#3}({#1})}
%\newcommand{\esubst}[2]{[#1/#2]}

\newcommand{\ren}[3]{({#1}\;{#2}) {#3}}
\newcommand{\renyx}[1]{\ren{y}{x}{#1}}

\renewcommand{\root}{\textsf{\tiny{r\,o\,o\,t}}}
\newcommand{\Rew}[2][]{\stackrel{#1}{\longrightarrow}_{#2}\;}
\newcommand{\Rewn}[2][*]{{\longrightarrow}^{#1}_{#2}\;}
\newcommand{\Rewplus}[2][+]{{\longrightarrow}^{#1}_{#2}\;}
\newcommand{\Rewsn}[2][*]{{\longleftrightarrow}^{#1}_{#2}\;}



==> Macros/old/Macros_1Logic.tex <==
%Syntax
%Kinds

\newcommand\Arr[2]{{#1}\rightarrow {#2}}

%Types
\newcommand\et{{\wedge}}
\newcommand\andP{{\wedge^+}}
\newcommand\andN{{\wedge^-}}
\newcommand\ou{{\vee}}
\newcommand\orP{{\vee^+}}
\newcommand\orN{{\vee^-}}
\newcommand\trueP{{\top^+}}
\newcommand\trueN{{\top^-}}
\newcommand\falseP{{\bot^+}}
\newcommand\falseN{{\bot^-}}
\newcommand\negP{{\neg^+}}
\newcommand\negN{{\neg^-}}
\newcommand\imp{{\Rightarrow}}

\newcommand\EX[3][]{\exists #2^{#1} #3}
\newcommand\FA[3][]{\forall #2^{#1} #3}

\newcommand{\non}[1]{{#1}^{\perp}}
\newcommand{\eqT}{\approx}


\newcommand{\varT}{\textsf{Var}^T}
\newcommand{\fall}[3][{}]{\forall{#2}^{#1}.{#3}}
\newcommand{\xists}[3][{}]{\exists{#2}^{#1}.{#3}}
%\newcommand{\et}[2]{{#1}\wedge {#2}}
%\newcommand{\ou}[2]{{#1}\vee {#2}}
%\newcommand{\impl}[2]{{#1}\arr {#2}}
\newcommand{\nega}[1]{\overline{#1}}
\newcommand{\lamb}[3]{\lambda{#2}^{#1}.{#3}}
\newcommand{\dual}[1]{{#1}^{\bot}}
\newcommand{\bidual}[1]{{#1}^{\bot\bot}}
\newcommand{\tridual}[1]{{#1}^{\bot\bot\bot}}

\newcommand\ex [3][]{{#2}^{#1}.#3}
%\newcommand\exT[3][]{{#2}^{#1}.#3}

\newcommand\xistscod[3][{}]{\exists^{\textsf{cod}}{#2}^{#1}.{#3}}
\newcommand{\etcod}[2]{{#1}\wedge^{\textsf{cod}} {#2}}
\newcommand{\oucod}[2]{{#1}\vee^{\textsf{cod}} {#2}}

% %\newcommand\andP{\otimes}
% %\newcommand\andN{\&}
% %\newcommand\orP{\oplus}
% %\newcommand\orN{\vee^-}
% %\newcommand\imp{\multimap}

%Terms
\newcommand\proji[2]{#1}
\newcommand\projii[2]{#2}


%%%%%%%%%%%%%%%%%%%%%%%%
% Chapter 3

\newcommand\Terms{\frak R}
\newcommand\Sorts{\frak S}

\newcommand\TermSubs{\frak P}
\newcommand\RCextend[1][]{;}
\newcommand\RClift[1]{{#1}^+}

\newcommand\tsubs[2]{#2\{#1\}}

\newcommand\SContexts{\frak G}
\newcommand\SCextend[1][]{;}
\newcommand\SCid[1]{\textsf{id}_{#1}}

\newcommand\DecompType[1][]{\mathcal D_{#1}}
\newcommand\SubsType[1][]{\bullet\bullet\bullet}

%\newcommand{\var}{\textsf{Var}}
\newcommand{\var}[1][]{\textsf{Var}^{#1}}

\newcommand\Contexts[1][]{\mathcal G_{#1}}
\newcommand\Cextend[1][]{;}
\newcommand\CSContext[1]{\Sigma_{#1}}

\newcommand{\Atms}{\mathcal At}
\newcommand{\Moles}{\mathcal Mo}

\newcommand{\Lit}{\mathcal L}
\newcommand{\Forms}{\mathcal F}
\newcommand{\Just}{\mathcal J}
\newcommand{\Data}{\mathcal P}
\newcommand{\PTerms}{\mathcal H}
\newcommand{\Decomp}{\mathcal S}

\newcommand{\Subs}{\bullet\bullet\bullet}



% SubstitutionsTypes
\newcommand\Drefute[1]{{\sim}#1}
\newcommand\Dand{,}
\newcommand\Dunit{\bullet}
\newcommand\Dex[3][]{{#1}.{#3}}

% Substitutions
\newcommand\Tunit{\bullet}
\newcommand\Tand{,}
\newcommand\Tex[3][]{{#2}^{#1}.{#3}}
\newcommand\THO[2][]{{#2}}

% Commands
\newcommand\cutc[2]{\{#1\star#2\}}
\newcommand\just[1]{\{#1\}}


%% \newcommand\support[1]{\textsf{supp}(#1)}
%% \newcommand\fresh[2]{#1\sharp#2}
%% \newcommand{\NamingConvs}{\mathcal N}

%% %\newcommand{\lamc}[4][{}{}]{{#2}^{\i #1}{#3}^{\ii #1}.{#4}}
%% %\newcommand\stac[2]{{#1}\cdot{{#2}}}
%% %\newcommand{\inj}[4][{}{}]{\lambda #2^{\proji #1}#3^{\projii #1}.{#4}}
%% %\newcommand{\switch}[1]{\bullet #1}

%% \newcommand{\Lamb}[3]{\Lambda{#2}^{#1}.{#3}}
%% \newcommand{\appl}[2]{\langle #1,#2\rangle}

%% \newcommand\down[1]{\downarrow\!#1}


%% \newcommand{\m}[3][{}]{\mu #2^{#1}\!.{#3}}
%%\newcommand{\mt}[3][{}]{\tilde\mu {#2}^{#1}.{#3}}

\newcommand{\Acc}[2][]{\textsf{Im}^{#1}(#2)}

% Example of classical logic

\newcommand\Ppos{\_^+}
\newcommand\Pneg{\_^-}
\newcommand\Ptrue{\bullet}
\newcommand\inj[2]{\textsf{inj}_{#1}{(#2)}}
\newcommand\paire[2]{({#1},{#2})}

\newcommand\project[2]{\pi_{#1}{(#2)}}
\newcommand\caseanal[2]{[{#1},{#2}]}
\newcommand\switchl[1]{{\curvearrowleft}{(#1)}}
\newcommand\switchr[1]{{\curvearrowright}{(#1)}}

\newcommand\flatten[1]{\overline{#1}}

\newcommand\lefths{\textsf{l}}
\newcommand\righths{\textsf{r}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Chapter 4
%Semantics:

\newcommand{\semK}[1]{[\![#1]\!]}
\newcommand{\swapK}[2]{\textsf{swap}_{#1}{#2}}

\newcommand{\sem}[2]{[\![#2]\!]_{#1}}
\newcommand{\semt}[1]{[\![#1]\!]}
% \newcommand\sem[2]{[#1]_{#2}}

\newcommand{\orth}[2]{{#1\mathrel{{\perp}}#2}}

\newcommand{\effac}[1]{\|{#1}\|}
\newcommand{\twt}{\mathcal{T}}

\newcommand{\mU}{\mathcal U}
\newcommand{\mV}{\mathcal V}

\newcommand{\fp}[2]{\Phi_{#1}{#2}}
\newcommand\LamC[1]{\Lambda\_.{#1}}
\newcommand\applC[1]{\appl{\_}{#1}}


==> Macros/old/Macros_2LJNJ.tex <==
%DERIVABILITY

% Types and Typing
\newcommand\arr{\hspace{-3pt}\rightarrow\hspace{-3pt}}
\newcommand\rto{\arr}
\renewcommand\>{\arr}

\newcommand\col{\unskip\colon}
\newcommand\XcolY[2]{#1\col#2}
\newcommand\varRead[2][]{#2_{|#1}}
\newcommand\getvar[3][]{#2_{|#1}=#3}


% Generic derivability symbol
\newcommand{\seqg}[3]{\mbox{$\ {#1}_{#2}^{#3}\ $}}

% ... with vdash and models and their negations
\newcommand{\seqf} [2][]{\seqg{\vdash}     {#1}{#2}}
\newcommand{\nseqf}[2][]{\seqg{\not\vdash} {#1}{#2}}
\newcommand{\satf} [2][]{\seqg{\models}    {#1}{#2}}
\newcommand{\nsatf}[2][]{\seqg{\not\models}{#1}{#2}}
\newcommand{\decf} [2][]{\seqg{\Vdash}    {#1}{#2}}
\newcommand{\ndecf}[2][]{\seqg{\not\Vdash}{#1}{#2}}

%Purely logical

\newcommand\DerF[4][]{{#2}\seqf[{#1}]{}{[#3]}{#4}}
\newcommand\Der[3][]{{#2}\seqf[{#1}]{}{#3}}

\newcommand\DertF[5][]{{#3}\seqf[{#1}]{#2}{[#4]}{#5}}
\newcommand\Dert[4][]{{#3}\seqf[{#1}]{#2}{#4}}

\newcommand\DerDec[4][]{{#3}\decf[{#1}]{#2}{#4}}

\newcommand\DerTF[4][]{{#2}\satf[{#1}]{}{[#3]}{#4}}
\newcommand\DerT[3][]{{#2}\satf[{#1}]{}{#3}}

%Per systems

\newcommand\DerDPLL[2] {{#1}\mbox{;}{#2}\seq}


%Rules

\newcommand\ax{\textsf{ax}}
\newcommand\cut{\textsf{cut}}
\newcommand\re{\hspace{4pt}\arr_{\textsf{elim}}}

\newcommand\weakening{\textsf{weak}}
\newcommand\contraction{\textsf{cont}}


%Proof-term Syntax

\newcommand\daggerL{\raise3pt\hbox{\rotatebox{-40}{$\dagger$}}}
\newcommand\daggerR{\raise0pt\hbox{\rotatebox{40}{$\dagger$}}}


\newcommand\letin[3]{\left\langle{#1}\dagger {#2}.{#3}\right\rangle}
\newcommand\ltin[1]{\{#1\}}
\newcommand\hole{[]}


% new for DPLL
%\newcommand{\seqgD}[4]{\mbox{$\ {#1}_{#2}^{#3}_(#4)\ $}}
%\newcommand{\seqfD}[2][]{\seqgD{\vdash}{#1}{#2}}
%end

%new for Theory
%\newcommand{\seqTh}[2][]{\seqg{\vdash_{\mathcal{T}}}{#1}{#2}}
%\newcommand{\seqThD}[2][]{\seqg{\vdash_{\mathcal{T}}^{\Delta_0}}{#1}{#2}} % for DPLL (for \Del_0)
% \newcommand{\seqThD}[2][]{\seqf[#1]\mathcal{T}}^{\mathcal P}}{#1}{#2}} % for DPLL \mathcal{P}
% \newcommand{\seqFOL}[2][]{\seqg{\vdash_{FOL}}{#1}{#2}} % First order Logic
% % end
% %new for Th
% \newcommand{\seqt}[1][]{\seqTh[#1]{}}
% \newcommand{\seqtD}[1][]{\seqThD[#1]{}}
% \newcommand{\seqFol}[1][]{\seqFOL[#1]{}}  %new for FOL
% %end


==> Macros/old/Macros_3CBV.tex <==
\newcommand\CPS{\textsf{CPS}}

%Moggi's lC
\newcommand\letinC[3]{\textsf{let }#2=#1\textsf{ in }{#3}}

\newcommand\bv{\beta_{\textsf V}}
\newcommand\ev{\eta_{\textsf V}}
\newcommand\evp{\eta'_{\textsf V}}


\newcommand\bl{{\textsf {B}}}
\newcommand\letC{{\textsf {let}}_{\textsf V}}
\newcommand\appleti{{\textsf {let}}_1}
\newcommand\appletii{{\textsf {let}}_2}
\newcommand\etalet{\eta_{\textsf {let}}}
\newcommand\letnesting{{\textsf {assoc}}}

%\newcommand\lCx{\lambda_{{\textsf C}\textsf{x}}}
\newcommand\lCb{\lambda_{{\textsf C}\beta}}
\newcommand\lCbe{\lambda_{{\textsf C}\beta\eta}}

%CPS-translations
\renewcommand\Re[1]{\mathcal{R}(#1)}
\newcommand\ReV[1]{\mathcal{R}_{\textsf V}(#1)}
\newcommand\Fi[1]{\mathcal{F}(#1)}
\newcommand\FiV[1]{\mathcal{F}_{\textsf V}(#1)}

\newcommand\Fis[2]{{#1}\colon_{\!\!\mathcal{F}}{#2}}
\newcommand\FisV[1]{{#1}^{\mathcal F}}
\newcommand\Rey[2]{{#1}\colon_{\!\!\mathcal{R}}{#2}}
\newcommand\ReyV[1]{{#1}^{\mathcal R}}

\newcommand\Fisback[1]{{#1}^{{\mathcal F}{\textsf {back}}}}
\newcommand\Fisbackname{{\mathcal F}{\textsf {back}}}


%Calculs CPS
\newcommand\lav{$\lambda_{\textsf {EvalArg}}$}
\newcommand\lContR{$\lambda^{\mathcal R}_{\CPS}$}
\newcommand\lContF{$\lambda^{\mathcal F}_{\CPS}$}
\newcommand\lContp{$\lambda_{\CPS}^+$}

\newcommand\lContRb{\lambda^{\mathcal R}_{\CPS\beta}}
\newcommand\lContRbe{\lambda^{\mathcal R}_{\CPS\beta\eta}}
\newcommand\lContFb{\lambda^{\mathcal F}_{\CPS\beta}}
\newcommand\lContFbe{\lambda^{\mathcal F}_{\CPS\beta\eta}}

\newcommand\lif[1]{\Uparrow{#1}}
\newcommand\lifname{\Uparrow}

%For later

\newcommand\lContfb{\lambda^{f}_{\CPS\beta}}
\newcommand\lContfbe{\lambda^{f}_{\CPS\beta\eta}}

\newcommand\nnot[1]{{#1}^{\bullet}}

\newcommand\liFf[1]{\uparrow{#1}}
\newcommand\liFfname{\uparrow}

\newcommand\cps[2]{{#1}\colon{#2}}
\newcommand\cpsV[1]{{#1}^{\dag}}

\newcommand\spc[1]{{#1}^{{\textsf {back}}}}
\newcommand\spcname{{(\_)}^{{\textsf {back}}}}

\newcommand\lContf{$\lambda^{f}_{\CPS}$}

\newcommand\lCont{\lambda_{\CPS}}

\newcommand\lConti{\lambda_{\textsf{cont}1}}
\newcommand\lContii{\lambda_{\textsf{cont2}}}

%To and from Moggi's C

\newcommand\Tii[1]{{#1}^{\sharp}}
\newcommand\Tiii[1]{{#1}^\natural}
\newcommand\Ti[1]{{#1}^\flat}

%\newcommand\Tiname{{(\_)}^\flat}
%\newcommand\Tiiname{{(\_)}^\sharp}
%\newcommand\Tiiiname{{(\_)}^\natural}


==> Macros/old/Macros_4DPLL.tex <==
\newcommand\emptylist{[\,]}
\newcommand\cons[2]{#1\mbox{$\colon\!\!\!\colon\!$}#2}


\newcommand\emptyenv{()}


\newcommand\backpoints[1]{[#1]}
\newcommand\backstrict[1]{\llbracket #1\rrbracket}
\newcommand\forget[1]{|#1|}



\newcommand\unsat{\textsf{UNSAT}}

\newcommand\DPLL{\textsf{DPLL}}
\newcommand\DPLLbj{\textsf{DPLL}$_{bj}$}
\newcommand\DPLLTh{\textsf{DPLL}($\mathcal T$)}
\newcommand\DPLLbjTh{\textsf{DPLL}$_{bj}$($\mathcal T$)}

\newcommand\nfDel[3][\mathcal T]{\textsf{nf}^{#1}_{#2}(#3)}

\newcommand\mSat[1]{\textsf{Sat} (#1)}

\newcommand\atm[1]{\textsf{lit} (#1)}
%\newcommand\atmCtxt[1]{\textsf{lit\_ctxt} (#1)}
\newcommand\atmCtxt[1]{{#1}_{\textsf{lit}}}

\newcommand\nSat[2]{\textsf{Sat}_{#1}{(#2)}}

\newcommand\pTree{\textsf{Partial proof tree}}

\newcommand\compat[2]{\textsf{cpt}(#1,#2)}

\newcommand\Init[1][]{\textsf{Init}_{#1}}
\newcommand\Release{\textsf{Release}}
\newcommand\Select{\textsf{Select}}
\newcommand\Store{\textsf{Store}}
\newcommand\Pol{\textsf{Pol}}

\renewcommand\sqin{\raise1pt\hbox{\large $\,\epsilon\,$}}

==> Macros/old/Macros_4LambdaI.tex <==
%lambda I

\renewcommand\corner[1]{\v{#1}}
\newcommand\wonalc{$\l^?$}
\newcommand\subanot[2]{#1\lhd{#2}}

\renewcommand\P[3]{\Pi {#1}^{#2}.{#3}}
\newcommand\lami[3]{\lambda {#1}^{#2}.{#3}}

\newcommand\dummy{\wp}
\renewcommand\i[1]{\textsf{i}({#1})}
\newcommand\iname{\textsf{i}}

\newcommand\typ{t}
\newcommand\betat{{\beta^{\typ}}}

\newcommand\pervar{\textsf{perp-var}}
\newcommand\perl{\textsf{perp}\lambda}
\newcommand\perlaa{\textsf{perp}\lambda^{\typ}_1}
\newcommand\perlab{\textsf{perp}\lambda^{\typ}_2}
\newcommand\perba{\textsf{perp}\beta_1}
\newcommand\perbb{\textsf{perp}\beta_2}
\newcommand\perbaa{\textsf{perp}\betat_1}
\newcommand\perbba{\textsf{perp}\betat_2}
\newcommand\perbca{\textsf{perp}\betat_3}
\newcommand\perpia{\textsf{perp}\Pi_1}
\newcommand\perpib{\textsf{perp}\Pi_2}

\newcommand\per{\rightsquigarrow}

\newcommand\RI[2]{{#1}\;\mathcal H\;{#2}}

\newcommand\GI[2]{{#1}\;\mathcal{G}\;{#2}}
\newcommand\Gax{\mathcal{G}\textsf{ax}}
\newcommand\Gvar{\mathcal{G}\textsf{var}}
\newcommand\Gl{\mathcal{G}\lambda}
\newcommand\Gla{\mathcal{G}\lambda^{\typ}}
\newcommand\Gba{\mathcal{G}\beta_1}
\newcommand\Gbb{\mathcal{G}\beta_2}
\newcommand\Gbaa{\mathcal{G}\betat_1}
\newcommand\Gbba{\mathcal{G}\betat_2}
\newcommand\Gweak{\mathcal{G}\textsf{weak}}
\newcommand\Gweaka{\mathcal{G}\textsf{weak1}}
\newcommand\Gweakb{\mathcal{G}\textsf{weak2}}
\newcommand\Gc{\mathcal{G}\textsf{c}}
\newcommand\Gpi{\mathcal{G}\textsf{$\Pi$}}

==> Macros/old/Macros_4SafeMin.tex <==
%PSN & Encodings to and from lambda=======================

\newcommand{\PSN}{{\textsf{PSN}}}


\renewcommand\H[1]{\textsf{H}({#1})}
\newcommand\Hname{\textsf{H}}
\newcommand\xtol[1]{\H{#1}}
\newcommand\xtolname{\Hname}

\newcommand\delambda[1][]{{\mathcal A}_{#1}}
\newcommand\alambda{{\mathcal B}}
\newcommand\dd[1]{\delambda(\alambda({#1}))}

\newcommand\kC[1]{{\delambda}_{\textsf{w}}{({#1})}}
\newcommand\kCCC[1]{{\delambda}{(#1)}}
\newcommand\kCC[2][]{{\delambda}_{#1}{(#2)}}
\newcommand\kCCname{{\delambda}}

\renewcommand\k[1]{\alambda{(#1)}}
\newcommand\kl[2]{\alambda^{#1}{(#2)}}
\newcommand\kname{{\mathcal B}}


%RPO encoding

\newcommand\polyx[1]{\overline{#1}}
\newcommand\polyxname{\overline {(\;)}}
\newcommand\polyxg[1]{\polyx{#1}}
\newcommand\polyxgname{\polyxname}


\newcommand\nb[1]{\sharp #1}

\newcommand\fo[1]{\polyx {#1}}
\newcommand\foe[1]{\polyx {#1}}
\newcommand\foename{\polyxname}

\newcommand\fot[1]{\polyx {#1}}
\newcommand\fotname{\polyxname}


\ignore{
\newcommand\polyx[1]{\mathcal P(#1)}
\newcommand\polyxname{\mathcal P}
}


%Safeness and minimality

\newcommand\safe[1]{\textsf{safe} {#1}}
\newcommand\minim[2]{\textsf{min}_{#1} #2}
\renewcommand\min[1]{\minim{}{#1}}

\newcommand{\unsafe}[1]{{\stackrel{\textsf{unsafe}}\longrightarrow}_{#1}\;}
\newcommand{\unsafen}[1]{{{\stackrel{\textsf{unsafe}}\longrightarrow}^{*}}_{#1}\;}
\newcommand{\unsafeplus}[1]{{{\stackrel{\textsf{unsafe}}\longrightarrow}^{+}}_{#1}\;}
\newcommand{\undafesn}[1]{{{\stackrel{\textsf{unsafe}}\longrightarrow}^{*}}_{#1}\;}


%Lambda x
\newcommand\lamp[3]{\lambda {#1}.{#3}}
\newcommand\cuti[4]{\langle{#2}/{#3}\rangle{#4}}

\newcommand\x{\textsf{x}}



==> Macros/old/Macros_5Llxr.tex <==
\newcommand\strict{basic}
\newcommand\expsub{substitution constructor}

%Rewriting specific===========================

\newcommand{\Sim}[1]{\sim_{#1}\;}
\newcommand{\Rewmod}[2]{\rightarrow_{#1/#2}\;}
\newcommand{\Rewmodn}[2]{\rightarrow^{*}_{#1/#2}\;}

\newcommand{\LRewplus}[1]{\; \mbox{}_{#1}^{+}{\longleftarrow}\;}
\newcommand{\LRew}[1]{\; \mbox{}_{#1}{\longleftarrow}}
\newcommand{\LRewn}[1]{\; {\mbox{}_{#1\,}}^{*}{\longleftarrow}}
\newcommand{\RLRewn}[1]{{\longleftrightarrow}^{*}_{#1}}
\newcommand{\RLRew}[1]{{\longleftrightarrow}_{#1}}


\newcommand{\ssubst}[3]{\subst{#1}{#3}{#2}}
%\newcommand{\isubst}[2]{\{ #1 \backslash #2 \} }



%Terms===========================

\renewcommand\t{\textsf{r}}
\newcommand\xt{\textsf{xr}}
\newcommand{\weak}[2]{\mathcal{W}_{#1}(#2)}
\newcommand{\app}[4]{#1\; #3}

\newcommand{\clos}[2]{#2 {#1}}
\newcommand{\trip}[3]{\cuti{}{#2} {#1}}

%\newcommand{\clos}[2]{#1\langle #2\rangle}
%\newcommand{\trip}[3]{#1 =_{#3} #2}
%\newcommand{\iclos}[2]{#1[#2]}
\newcommand{\con}[4]{\mathcal{C}_{#1}^{#2\,|\,#3}(#4)}

\newcommand{\weakapp}[5]{\weak {#1}{\app {#2}{} {#4}{}}}

\newcommand{\wf}{\mbox{ \textsf{linear}}}

%Equations======================
\newcommand{\ac}{\textsf{A}_{\textsf{c}}}
\newcommand{\ccu}{\textsf{C}_{\textsf{c}}}
\newcommand{\ccd}{\textsf{P}_{\textsf{c}}}
\newcommand{\cw}{\textsf{P}_{\textsf{w}}}
\newcommand{\com}{\textsf{P}_{\textsf{s}}}
\newcommand{\cs}{\textsf{P}_\textsf{cs}}


%Rules============================

\newcommand\Abs{\textsf{Abs}}
\newcommand\Appi{\textsf{App1}}
\newcommand\Appii{\textsf{App2}}
\newcommand\Var{\textsf{Var}} 
\newcommand\Weaki{\textsf{Weak1}}
\newcommand\Weakii{\textsf{Weak2}}
\newcommand\Cont{\textsf{Cont}}
\newcommand\Comp{\textsf{Comp}}
\newcommand\WAbs{\textsf{WAbs}}
\newcommand\WAppi{\textsf{WApp1}}
\newcommand\WAppii{\textsf{WApp2}}
\newcommand\WSubs{\textsf{WSubs}} 
\newcommand\Merge{\textsf{Merge}}
\newcommand\Cross{\textsf{Cross}}
\newcommand\CAbs{\textsf{CAbs}}
\newcommand\CAppi{\textsf{CApp1}} 
\newcommand\CAppii{\textsf{CApp2}} 
\newcommand\CSubs{\textsf{CSubs}}

%Translation=================

\newcommand{\ord}[1]{{#1}}

%sn-x=========================
\newcommand\multip[2]{\mathcal M_{#1}({#2})}
\newcommand\Tcomplex[1]{\mathcal {T}\!\textsf{x} ({#1})}
\newcommand\pol[1]{\mathcal P({#1})}
\newcommand\polname{\mathcal P}

==> Macros/old/Macros_6G3.tex <==
%Strategies
\newcommand\princ{{\textsf{princ}}}
\newcommand\gauche{\textsf{left}}
\newcommand\droite{\textsf{right}}

\newcommand\simpl{{\textsf{s}}}
\newcommand\SI{{\textsf{SI}}}
\newcommand\KK{{\textsf{KK}}}
\newcommand\JC{{\textsf{JC}}}

\newcommand\CBV{\textsf{CBV}}
\newcommand\CBN{\textsf{CBN}}
\newcommand\CBVs{\textsf{CBV}_{\textsf{simple}}}
\newcommand\CBNs{\textsf{CBN}_{\textsf{simple}}}
\newcommand\CB{\textsf{CB}}
\newcommand\equCBV{\equiv_{\CBV}}
\newcommand\equCBN{\equiv_{\CBN}}

\newcommand\clas{\equiv}
\newcommand\mogo{\textsf{sc}}
\newcommand\quot{\textsf{nd}}

\newcommand\purq{\textsf{pur-q}}
\newcommand\purt{\textsf{pur-t}}
\newcommand\purGp{\textsf{pur}\Giiii'}
\newcommand\purGiv{\textsf{pur}\Giv}


%lambdabar

\newcommand\SVar{{\mathcal X}}
\newcommand\STerms{{\mathcal T}}
\newcommand\SLists{{\mathcal L}}

\newcommand\TSVar{{\mathcal Y}}
\newcommand\PSVar{{\mathcal X}}
\newcommand\TS{{\mathcal P}}
\newcommand\PSTerms{{\mathcal T}}
\newcommand\PSLists{{\mathcal L}}


\newcommand\cont[2]{{#1}\;{#2}}

\newcommand\el{[]}
\newcommand\conc[2]{{#1}@{#2}}
\newcommand\st[2]{{#1}\cdot{#2}}

%Typing
\newcommand\contr[1]{\textsf{select}_{#1}}

\newcommand\Air{\rightarrow\textsf{r}}
\newcommand\Ail{\rightarrow\textsf{l}}


%Term reduction rules
\newcommand\B{\textsf{B}}
\newcommand\Ai{\textsf{A1}}
\newcommand\Aii{\textsf{A2}}
\newcommand\Aiii{\textsf{A3}}
\newcommand\Bi{\textsf{B1}}
\newcommand\Bii{\textsf{B2}}
\newcommand\Biii{\textsf{B3}}
\newcommand\Ci{\textsf{C1}}
\newcommand\Cii{\textsf{C2}}
\newcommand\Ciii{\textsf{C3}}
\newcommand\Civ{\textsf{C4}}
\newcommand\Cv{\textsf{C5}}
\newcommand\Cvi{\textsf{C6}}
\newcommand\Cvii{\textsf{C7}}
\newcommand\Cviii{\textsf{C8}}
\newcommand\Di{\textsf{D1}}
\newcommand\Dii{\textsf{D2}}
\newcommand\Diii{\textsf{D3}}
\newcommand\Div{\textsf{D4}}
%\newcommand\Ei{\textsf{E}}
%\newcommand\Fi{\textsf{F}}

\newcommand\As{\textsf{As}}
\newcommand\Bs{\textsf{Bs}}
\newcommand\Cs{\textsf{Cs}}
\newcommand\CGs{\textsf{Cs}_{\textsf G}}
\newcommand\Ds{\textsf{Ds}}
\newcommand\Es{\textsf{E}}

==> Macros/old/Macros_7G4.tex <==
\def\ijcar{}
\def\journal{\ignore}
%=================================================

\newcommand{\Lveerto}{\mbox{$L\!\vee\!\rto$}}

\newcommand{\AB}{A\rto B}
\newcommand{\BA}{B\rto A}

\newcommand{\BC}{B\rto C}

\newcommand{\ABC}{(\AB) \rto C}
\newcommand{\CD}{C\rto D}
\newcommand{\DB}{D\rto B}
%\newcommand{\CB}{C\rto B}
\newcommand{\FG}{F\rto G}
\newcommand{\GH}{G\rto H}
\newcommand{\CDB}{(\CD)\rto B}
\newcommand{\FGH}{(\FG)\rto H}

\newcommand{\dec}[2]{\mbox{${#1}\!\colon\!{#2}$}}
\newcommand{\vA}{\mbox{$\dec{v}{A}$}}
\newcommand{\vB}{\mbox{$\dec{v}{B}$}}
\newcommand{\uC}{\mbox{$\dec{u}{C}$}}
\newcommand{\vC}{\mbox{$\dec{v}{C}$}}
\newcommand{\wA}{\mbox{$\dec{w}{A}$}}
\newcommand{\wB}{\mbox{$\dec{w}{B}$}}
\newcommand{\wC}{\mbox{$\dec{w}{C}$}}
\newcommand{\wD}{\mbox{$\dec{w}{D}$}}
\newcommand{\wE}{\mbox{$\dec{w}{E}$}}
\newcommand{\xA}{\mbox{$\dec{x}{A}$}}
\newcommand{\xB}{\mbox{$\dec{x}{B}$}}
\newcommand{\xC}{\mbox{$\dec{x}{C}$}}
\newcommand{\yA}{\mbox{$\dec{y}{A}$}}
\newcommand{\yB}{\mbox{$\dec{y}{B}$}}
\newcommand{\yC}{\mbox{$\dec{y}{C}$}}
\newcommand{\yD}{\mbox{$\dec{y}{D}$}}
\newcommand{\yE}{\mbox{$\dec{y}{E}$}}
\newcommand{\zA}{\mbox{$\dec{z}{A}$}}
\newcommand{\zB}{\mbox{$\dec{z}{B}$}}
\newcommand{\zC}{\mbox{$\dec{z}{C}$}}
\newcommand{\zD}{\mbox{$\dec{z}{D}$}}
\newcommand{\zE}{\mbox{$\dec{z}{E}$}}
\newcommand{\MA}{\mbox{$\dec{M}{A}$}}
\newcommand{\MB}{\mbox{$\dec{M}{B}$}}
\newcommand{\MD}{\mbox{$\dec{M}{D}$}}
\newcommand{\ME}{\mbox{$\dec{M}{E}$}}
\newcommand{\NA}{\mbox{$\dec{N}{A}$}}
\newcommand{\NB}{\mbox{$\dec{N}{B}$}}
\newcommand{\ND}{\mbox{$\dec{N}{D}$}}
\newcommand{\NE}{\mbox{$\dec{N}{E}$}}


                    
\ignore{
\newcommand{\esapp}[4]{\langle\!\langle #1/#2, #3,#4  \rangle    \!   \rangle}
\newcommand{\esappt}[3]{\langle\!\langle #1/#2, #3  \rangle    \!   \rangle}
\newcommand{\tesapp}[1]{\langle\!\langle #1 \rangle  \! \rangle}
\newcommand{\nomtesapp}{\langle\!\langle ~ \rangle \!\rangle}
\newcommand{\tsapp}[1]{\{\!\{ #1 \}  \! \}}
\newcommand{\nomtsapp}{\{ \! \{ ~ \} \! \}}
\newcommand{\sapp}[3]{\{\!\{#1/#2,#3 \}\! \}}
\newcommand{\ce}[2]{[\![#1/#2]\!]}
\newcommand{\nomcut}{cut}
\newcommand{\tcut}[2]{cut(#1,#2)}
\newcommand{\la}[4]{{\tt app}(#1,#2,#3.#4)}
\newcommand{\rew}{\rightarrow}
%\newcommand{\tra}[1]{{\cal T}(#1)}
\newcommand{\tra}[1]{\overline{#1}}
%\newcommand{\tce}[4]{[\![#4]\!]_{#1,#2,#3}}
\newcommand{\tce}[2]{[\![#2]\!]_{#1}}
\newcommand{\nomtce}{[\![~]\!]_{A}}
\newcommand{\tes}[2]{[#2]_{#1}}
\newcommand{\nomtes}{[~]_{A}}



\newcommand{\spred}{\triangleright}
\newcommand{\pair}[2]{\langle #1,#2\rangle}
\newcommand{\triple}[3]{\langle #1,#2,#3\rangle}
\newcommand{\app}[2]{app(#1,#2)}
\newcommand{\tapp}[3]{app(#2,#3)_{#1}}
\newcommand{\nomtapp}{app_{A}}
\newcommand{\msep}{\hspace{.5cm}}
}

\newcommand{\lam}[2]{\lambda {#1}.{#2}}
\newcommand{\leftz}[4]{#1[#2,#3.#4]}
\newcommand{\leftr}[6]{#1[#2.#3.#4,#5.#6]}
\newcommand{\inv}[3]{{\tt inv}(#1,#2.#3)}
\newcommand{\ninv}{{\tt inv}}
\newcommand{\inva}[2]{{\tt inva}(#1,#2)}
\newcommand{\invz}[3]{{\tt inv}(#1,#2.#3)}
\newcommand{\ninvz}{{\tt inv}}
\newcommand{\invr}[3]{{\tt inv}(#1,#2.#3)}

\newcommand{\type}[1]{\widehat{#1}}
%\newcommand{\of}[2]{#1 \; {\tt of }\; #2}
\newcommand{\of}[2]{{\tt of}(#1,#2)}
\newcommand{\nof}{{\tt of}}
\newcommand{\Of}{O\! f}
\newcommand{\Inv}{Inv}
\newcommand{\genax}[2]{{\tt Ax}(#1,#2)}
\newcommand{\decomp}[4]{{\tt dec}(#1,#2,#3.#4)}
\newcommand{\ndecomp}{{\tt dec}}
%\renewcommand{\ar}[3]{(#1 \rto #2) \rto #3}

\newcommand{\Cut}[3]{\letin {#1}{#2}{#3}}
\newcommand{\ncut}{{\tt cut}}

%========================
%Rewrite rules

\newcommand\decri{\textsf{d}1}
\newcommand\decrii{\textsf{d}2}
\newcommand\decriii{\textsf{d}3}
\newcommand\decriv{\textsf{d}4}
\newcommand\decrv{\textsf{d}5}
\newcommand\decrvi{\textsf{d}6}
\newcommand\decrvii{\textsf{d}7}
\newcommand\decrviii{\textsf{d}8}

\newcommand\cutri{\textsf{c}1}
\newcommand\cutrii{\textsf{c}2}
\newcommand\cutriii{\textsf{c}3}
\newcommand\cutriv{\textsf{c}4}
\newcommand\cutrv{\textsf{c}5}
\newcommand\cutrvi{\textsf{c}6}
\newcommand\cutrvii{\textsf{c}7}
\newcommand\cutrviii{\textsf{c}8}
\newcommand\cutrix{\textsf{c}9}

\ignore{
\newcommand\cutrx{\textsf{c}{10}}
\newcommand\cutrxi{\textsf{c}{11}}
\newcommand\cutrxii{\textsf{c}{12}}
\newcommand\cutrxiii{\textsf{c}{13}}
\newcommand\cutrxiv{\textsf{c}{14}}
\newcommand\cutrxv{\textsf{c}{15}}
\newcommand\cutrxvi{\textsf{c}{16}}
}

\ignore{
\newcommand\cutri{a}
\newcommand\cutrii{b}
\newcommand\cutriii{c}
\newcommand\cutriv{d}
\newcommand\cutrv{e}
\newcommand\cutrvi{f}
\newcommand\cutrvii{g}
\newcommand\cutrviii{\pi}
\newcommand\cutrix{\phi}
}
\newcommand\cutrx{\textsf{A}}
\newcommand\cutrxi{\textsf{B}}
\newcommand\cutrxii{\textsf{C}}
\newcommand\cutrxiii{\textsf{D}}
\newcommand\cutrxiv{\textsf{E}}
\newcommand\cutrxv{\textsf{F}}
\newcommand\cutrxvi{\textsf{G}}


\newcommand\invi{\textsf{i}1}
\newcommand\invii{\textsf{i}2}
\newcommand\inviii{\textsf{i}3}
\newcommand\inviv{\textsf{i}4}
\newcommand\invv{\textsf{i}5}
\newcommand\invvi{\textsf{i}6}
\newcommand\invvii{\textsf{i}7}
\newcommand\invviii{\textsf{i}8}

\newcommand\ofi{\textsf{o}1}
\newcommand\ofii{\textsf{o}2}
\newcommand\ofiii{\textsf{o}3}
\newcommand\ofiv{\textsf{o}4}

\newcommand{\lz}{L0 \rto}
\newcommand{\lrr}{L \rto\rto}

\ignore{
\newcommand{\lzn}{Lb}
\newcommand{\lrrn}{Li}
}
\newcommand{\lzn}{\textsf{I}}
\newcommand{\lrrn}{\textsf{K}}
\newcommand{\foA}{\textsf{I}}
%\newcommand{\fo}{\star}
\newcommand{\foI}{\textsf{J}}
\newcommand{\foO}{\textsf{J}}
\newcommand{\fodec}[1]{\textsf{D}^{#1}}
\newcommand{\foCut}[1]{\textsf{C}^{#1}}


\newcommand{\oid}{{\sf{ivdc}}}
\newcommand{\oidgs}{{\sf{ivdcgs}}}
\newcommand{\gs}{{\sf{gs}}}
\newcommand{\cegs}{{\sf{cegs}}}
\newcommand{\rs}{{\sf{rs}}}
\newcommand{\cers}{{\sf{cers}}}
\newcommand{\ars}{{\sf{ars}}}
\newcommand{\cears}{{\sf{cears}}}
\newcommand{\cbn}{{\sf{cbn}}}
\newcommand{\cecbn}{{\sf{cecbn}}}
\newcommand{\cbv}{{\sf{cbv}}}
\newcommand{\cecbv}{{\sf{cecbv}}}

\newcommand{\pr}{Principal}
\newcommand{\np}{Non-Principal}
\newcommand{\na}{Non-Auxiliary}
\newcommand{\au}{Auxiliary}

\def\kindi{\textsf{Kind}_1}
\def\kindii{\textsf{Kind}_2}
\def\kindiii{\textsf{Kind}_3}

%\def\myitem{\vspace{.5cm}\item}

\def\derivable#1{\infer{#1}{\ldots}}
\def\parag{}


==> Macros/old/Macros_8PTSC.tex <==
\newcommand\SCons{{\mathcal S}}

\newcommand\RSTerms{{\mathcal Z}}
\newcommand\K{\mbox{$\Box$}}
\newcommand\T{\star}
\newcommand\Rel{{\mathcal R}}
\newcommand\Sort{{\mathcal A}}

\newcommand\xsubst{\textsf{xsubst}}

%Typing======================================
\newcommand\emptyenv{[]}
\newcommand\conv{\Rewsn{\B\x}}


\newcommand\DPTSC{\vdash_{\PTSC}}

\renewcommand\wf[1][\PTSC]{\hspace{5 pt}\textsf{wf}_{#1}}
%Previous def in Part1/Llxr_Macros



\newcommand\empt{\textsf{empty}}
\newcommand\extend{\textsf{extend}}
\newcommand\Ttyped{\textsf{sorted}}
\newcommand\Picons{\Pi\textsf{wf}}
\newcommand\Pir{\Pi\textsf{r}}
\newcommand\Pil{\Pi\textsf{l}}
\newcommand\convr{\textsf{conv}_r}
\newcommand\convl{\textsf{conv}_l}

\newcommand\subenv{\sqsubseteq}

%PTS==================================
\newcommand\DPTS{\vdash_{\PTS}}
\newcommand\DeriCoC[3]{{#1}\DPTS {#2}\col{#3}}


==> Macros/old/Macros_9DB.tex <==
%Sequent calculus of constructions

\newcommand\PTSCdb{\PTSC_{\sf{db}}}
\newcommand\PTSCi{\PTSC_{\sf{imp}}}

\newcommand\STermsdb{{\mathcal T}_{\sf{db}}}
\newcommand\SListsdb{{\mathcal L}_{\sf{db}}}

\newcommand\Pdb[3]{\Pi^{#2}{#3}}
\newcommand\lamidb[3]{\lambda^{#2}{#3}}
\newcommand\liftdb[3]{U^{#1}_{#2}{(#3)}}

\newcommand\cutjdb[4]{{#4}\{\hspace{-3pt}\{{{#3}\!\leftarrow\!{#2}}\}\hspace{-3pt}\}}
\newcommand\eln{{[\!]}}
\newcommand\appli[2]{#1(#2)}

\newcommand\compsup[1]{\overline{\sf{im}}(#1)}

\newcommand\cogg[2]{\pi^{#1}{(#2)}}
\newcommand\coggg[2]{\rho^{#1}{(#2)}}
\newcommand\ccdb[2]{{#2},{#1}}
\newcommand\DBname[2]{\overline{#2}^{\,#1}}
\newcommand\nameDB[2]{\underline{#2}_{\,#1}}
\newcommand\cofinG[1]{\phi_{#1}}



%Term reduction rules
\newcommand\Bdb{\textsf{B}_{\sf{db}}}
\newcommand\Aidb{\textsf{A1}_{\sf{db}}}
\newcommand\Aiidb{\textsf{A2}_{\sf{db}}}
\newcommand\Aiiidb{\textsf{A3}_{\sf{db}}}
\newcommand\Bidb{\textsf{B1}_{\sf{db}}}
\newcommand\Biidb{\textsf{B2}_{\sf{db}}}
\newcommand\Biiidb{\textsf{B3}_{\sf{db}}}
\newcommand\Bivdb{\textsf{B4}_{\sf{db}}}
\newcommand\Cidb{\textsf{C1}_{\sf{db}}}
\newcommand\Ciidb{\textsf{C2}_{\sf{db}}}
\newcommand\Ciiidb{\textsf{C3}_{\sf{db}}}
\newcommand\Ciiiidb{\textsf{C3'}_{\sf{db}}}
\newcommand\Civdb{\textsf{C4}_{\sf{db}}}
\newcommand\Cvdb{\textsf{C5}_{\sf{db}}}
\newcommand\Cvidb{\textsf{C6}_{\sf{db}}}
\newcommand\Cviidb{\textsf{C7}_{\sf{db}}}
\newcommand\Cviiidb{\textsf{C8}_{\sf{db}}}
\newcommand\Didb{\textsf{D1}_{\sf{db}}}
\newcommand\Diidb{\textsf{D2}_{\sf{db}}}
\newcommand\Diiidb{\textsf{D3}_{\sf{db}}}
\newcommand\Divdb{\textsf{D4}_{\sf{db}}}

\newcommand\Asdb{\textsf{As}_{\sf{db}}}
\newcommand\Bsdb{\textsf{Bs}_{\sf{db}}}
\newcommand\Csdb{\textsf{Cs}_{\sf{db}}}
\newcommand\Dsdb{\textsf{Ds}_{\sf{db}}}

\newcommand\xdb{\textsf{x}_{\sf{db}}}

\newcommand\Alldb{\Bdb\xdb}


%Typing

\newcommand\DeriTIdbf[3]{\Deri[{\sf{TS}}_{\sf{db}}]{#1}{#2}{\equiv\! #3}}
\newcommand\DeriTIdbsf[4]{\Deris[{\sf{TS}}_{\sf{db}}]{#1}{#2}{#3}{\equiv\! #4}}
\newcommand\DeriTIdb[3]{\Deri[{\sf{TS}}_{\sf{db}}]{#1}{#2}{#3}}
\newcommand\DeriTIdbs[4]{\Deris[{\sf{TS}}_{\sf{db}}]{#1}{#2}{#3}{#4}}
\newcommand\wfTIdb{\hspace{5 pt}\textsf{wf}_{\sf{TS}_{\sf{db}}}}

\newcommand\TIdb{{\sf{TS}}_{\sf{db}}}
\newcommand\PSdb{{\sf{PS}}_{\sf{db}}}

\newcommand\DeriPSdb[3]{\Deri[{\sf{PS}}_{\sf{db}}]{#1}{#2}{#3}}
\newcommand\DeriPSdbs[4]{\Deris[{\sf{PS}}_{\sf{db}}]{#1}{#2}{#3}{#4}}


==> Macros/old/Macros_9Enumeration.tex <==
\ignore{
\newcommand\enum[5]{#2\sep #3\Longrightarrow #4\sep #5}
\newcommand\enums[6]{#2;#3\sep #4\Longrightarrow #5\sep #6}
}

\newcommand\enum[5]{\Deri{#2}{#4}{#3}\sep {#5}}
\newcommand\enums[6]{\Deris{#2}{#3}{#5}{#4}\sep {#6}}
\newcommand\goals[2]{#1\Longrightarrow #2}

\newcommand\PE{\textsf{PE}}

\newcommand\enumPS[5]{\Derip{\PE}{#2}{#4}{#3}\sep {#5}}
\newcommand\enumPSs[6]{\Derip{\PE}{#2;#3}{#5}{#4}\sep {#6}}
\newcommand\goalsPS[2]{#1\Longrightarrow_{\PE} #2}


\newcommand\constr[3]{#2\stackrel{#1}\longleftrightarrow #3}


==> Macros/old/Macros_9ProofSearch.tex <==
%Proof search


\newcommand\DPS{\vdash_{\textsf{PS}}}
\newcommand\PSS{\textsf{PS}}


\newcommand\DeriPS[3]{{#1}\DPS {#2}\col{#3}}
\newcommand\DeriPSs[4]{{#1};{#2}\DPS {#3}\col{#4}}

\newcommand\TtypedPS{\textsf{sorted}_\textsf{PS}}
\newcommand\contrs[1]{\textsf{sel.}_{#1}}
\newcommand\axPS{\textsf{ax}_\textsf{PS}}
\newcommand\PiconsPS{\Pi\textsf{wf}_\textsf{PS}}
\newcommand\PirPS{\Pi\textsf{r}_\textsf{PS}}
\newcommand\PilPS{\Pi\textsf{l}_\textsf{PS}}



==> Macros/old/Macros_9Tsynth.tex <==
%TI

\newcommand\Deric[3]{\Deri{#1}{#2}{\equiv\! #3}}
\newcommand\Derics[4]{\Deris{#1}{#2}{#3}{\equiv\! #4}}



\newcommand\DeriTIf[3]{\Deri[{\textsf{TS}}]{#1}{#2}{\equiv\! #3}}
\newcommand\DeriTIsf[4]{\Deris[{\textsf{TS}}]{#1}{#2}{#3}{\equiv\! #4}}
\newcommand\DeriTI[3]{\Deri[{\textsf{TS}}]{#1}{#2}{#3}}
\newcommand\DeriTIs[4]{\Deris[{\textsf{TS}}]{#1}{#2}{#3}{#4}}
\newcommand\wfTI{\hspace{5 pt}\textsf{wf}_{\textsf{TS}}}

\newcommand\extendTI{\textsf{extend}_\textsf{TS}}
\newcommand\axTI{\textsf{ax}_\textsf{TS}}
\newcommand\PiconsTI{\Pi\textsf{wf}_\textsf{TS}}
\newcommand\PirTI{\Pi\textsf{r}_\textsf{TS}}
\newcommand\PilTI{\Pi\textsf{l}_\textsf{TS}}

\newcommand\convp{\Rewsn{\B\x}}

\newcommand\expimp[1]{\Downarrow\!(#1)}
\newcommand\expimpname{\Downarrow}
\newcommand\TI{\textsf{TS}}

==> Macros/old/Macros_DPLL.tex <==
\newcommand\emptylist{[\,]}
\newcommand\cons[2]{#1\mbox{$\colon\!\!\!\colon\!$}#2}


\newcommand\emptyenv{()}


\newcommand\backpoints[1]{[#1]}
\newcommand\backstrict[1]{\llbracket #1\rrbracket}
\newcommand\forget[1]{|#1|}



\newcommand\unsat{\textsf{UNSAT}}

\newcommand\DPLL{\textsf{DPLL}}
\newcommand\DPLLbj{\textsf{DPLL}$_{bj}$}
\newcommand\DPLLTh{\textsf{DPLL}($\mathcal T$)}
\newcommand\DPLLbjTh{\textsf{DPLL}$_{bj}$($\mathcal T$)}

\newcommand\nfDel[3][\mathcal T]{\textsf{nf}^{#1}_{#2}(#3)}

\newcommand\mSat[1]{\textsf{Sat} (#1)}

\newcommand\atm[1]{\textsf{lit} (#1)}
%\newcommand\atmCtxt[1]{\textsf{lit\_ctxt} (#1)}
\newcommand\atmCtxt[1]{{#1}_{\textsf{lit}}}

\newcommand\nSat[2]{\textsf{Sat}_{#1}{(#2)}}

\newcommand\pTree{\textsf{Partial proof tree}}

\newcommand\compat[2]{\textsf{cpt}(#1,#2)}

\newcommand\Init[1][]{\textsf{Init}_{#1}}
\newcommand\Release{\textsf{Release}}
\newcommand\Select{\textsf{Select}}
\newcommand\Store{\textsf{Store}}
\newcommand\Pol{\textsf{Pol}}

\renewcommand\sqin{\raise1pt\hbox{\large $\,\epsilon\,$}}

==> Macros/old/Macros_PMT.tex <==
% \newcommand\Theory[2][\mathcal T]{{#1}(#2)}
% \newcommand\separ{{\bf\ |\ }}


\newcommand\LKDPLL{\textsf{LK}${}_{\textsf{DPLL}}$}
\newcommand\LKDPLLc{\textsf{LK}${}^c_{\textsf{DPLL}}$}

% new add for theory
\newcommand\LKDPLLTh[1][\strut]{\textsf{LK}${}_{\textsf{DPLL}}$($#1$)}
\newcommand\LKDPLLThc[1][\strut]{\textsf{LK}${}^c_{\textsf{DPLL}}$($#1$)}
% new extending lkbpllth system
\newcommand\LKDPLLThp[1][\strut]{\textsf{LK}${}_{\textsf{DPLL}^{+}}$($#1$)}

%\newcommand\LKp{\textsf{LK}$^p$}  just now
\newcommand\LKp{\textsf{LK}$^p$}
\newcommand\LKTh[1][\mathcal T]{\textsf{LK}($#1$)}
\newcommand\LKThp[1][\mathcal T]{\textsf{LK}$^p$($#1$)}
\newcommand\LKThpc[1][\mathcal T]{\textsf{LK}${}^p_{\textsf{c}}$($#1$)}

\newcommand\size[1]{\sharp(#1)}

